No-Regret Caching with Noisy Request Estimates

Online learning algorithms have been successfully used to design caching policies with regret guarantees. Existing algorithms assume that the cache knows the exact request sequence, but this may not be feasible in high load and/or memory-constrained scenarios, where the cache may have access only to sampled requests or to approximate requests' counters. In this paper, we propose the Noisy-Follow-the-Perturbed-Leader (NFPL) algorithm, a variant of the classic Follow-the-Perturbed-Leader (FPL) when request estimates are noisy, and we show that the proposed solution has sublinear regret under specific conditions on the requests estimator. The experimental evaluation compares the proposed solution against classic caching policies and validates the proposed approach under both synthetic and real request traces.

==> Old_approach.tex <==
%\subsection{FPL with noisy costs}
\begin{algorithm}[t]
\KwIn{Set of decisions $\mathcal{X}$; Time Horizon $T$; $\hat R, \; \hat A, \; D$}
\KwOut{Sequence of decisions: $\{\mathbf{x}_t\}_{1}^{T}$}

$\eta \gets \sqrt{\frac{\hat R\cdot \hat A \cdot T}{D}}$ \\ 
$\hat{\textbf{costs}} \gets  0$ ,  \\ 
\For{round $t=1,2,...,T$}{
$\boldsymbol{\gamma}_t \sim \textbf{Unif}\left(\left[0, \eta\right]^{N}, \mathbb{I}_{N\times N}\right)$ \\
$\mathbf{x}_t \gets M(\hat{\textbf{costs}} +  \boldsymbol{\gamma}_t)$ \\ 
Observe $\hat{\mathbf{r}}_{t}$ \\
$\hat{\textbf{costs}} \gets \hat{\textbf{costs}} + \mathbf{\hat{r}}_t$
}
\caption{Noisy-Follow-the-Perturbed-Leader with Uniform Noise (NFPL)}
\label{alg:NFPL}
\end{algorithm}




In this section, we introduce the Noisy-Follow-the-Perturbed-Leader (NFPL) algorithm, which  utilizes noisy estimates of the requests, $\mathbf{\hat r}_t$, rather than the actual requests $\mathbf{r}_t$. Our analysis herein is not confined to the caching scenario discussed in Section~\ref{sec:bacground}. Instead, it is applicable to any situation where the agent incurs costs represented by the equation $\scalar{\mathbf{r}_t}{\mathbf{x}_t}$.
% $\scalar{\mathbf{\hat r}_t}{\mathbf x_t}$.  %Y: I think it should be r_t 

We assume that the vector  $\mathbf{\hat r}_t$ is an unbiased estimator of $\mathbf{r}_t\in \mathcal{\bar B}$ with support $\mathcal{\hat B}$ and  bounded $l_1$ norm, i.e.,
%Our main contribution is proposing a more general version of the FPL algorithm where we do not have necessarily access to the exact cost vector, $r_t$, but only to its estimation: $\hat r_t$. $\hat r_t$ is an unbiased estimator of $r_t$ with bounded $l_1$ norm for every realization, i.e. 
\begin{align}
   \E{\mathbf{\hat r}_t} = \mathbf{r}_t , \; \exists \hat A \in \mathbb{R}^+ \; \text{s.t.} \; \sup_{\mathbf{\hat r} \in \mathcal{\hat B}} \norm{\mathbf{\hat r} }_1 \leq \hat A\ ,
\end{align}
%G: we could try to improve the names of the constants. For me it would be natural to have R for the bound on the requests and perhaps C for the scalar product r x which corresponds to the cost.
where $\norm{r}_1 = \sum_{i=1}^{N} |\mathbf{r}_i|$.
% and $\mathcal{\hat B} \subseteq \mathbb{R}^N$ is the set of all the realizations of every possible vector in the cost set $\bar{\mathcal{B}}$.
% %Y I think this sentence is maybe unnecessary, because Giovanni already mentioned that \hat B is the support of the random variable so .. 
%all $\mathbf{r} \in \bar{\mathcal{B}}$, where $\bar{\mathcal{B}}$ is the set of all costs. %$\mathcal{\hat B} = \{\mathbf{\hat r}_t(\omega) : \omega \in \Omega\}$ where $\Omega$ is the set of all the realizations of $\mathbf{\hat r}_t$. 
To clearly describe the algorithm we also need to introduce the definition of the upper bound of the cost, and the diameter of the decision set $\mathcal{X} \subseteq \mathbb{R}^N$ as
\begin{align}
    &\hat R = \sup_{\mathbf{x}\in \mathcal{X}, \mathbf{r} \in \mathcal{\hat{B}}} \scalar{\mathbf{r}}{\mathbf{x}}\ ,\\
    %G: \bar{\hat{B}} is not defined, should it be \hat{B}?  % Y: Yes 
    &D= \sup_{\mathbf{x},\mathbf{y} \in \mathcal{X}} \norm{\mathbf{x}-\mathbf{y}}_{1}\ .
%    &A = \sup_{r\in \bar{\mathcal{B}}} \norm{r}_{1} 
\end{align}

We highlight that NFPL is not specific just to online caching, but it can deal with any general online linear learning problem. %Indeed, as described in Algorithm~\ref{alg:NFPL}, NFPL receives in input the set of decisions $\mathcal{X}$ that can be any compact subset of $\mathbb{R}^N$ with $l_1$ diameter $D$. %; iii) the upper bound $A$ on the norm of any realization of the request estimator; iv) the upper bound $R$ on the cost and v) the diameter $D$ of the decision set. 
As described in Algorithm~\ref{alg:NFPL}, NFPL follows in the footsteps of FPL with uniform noise, but considers the estimation from $\mathbf{\hat r}_t$ instead of the real cost vector $\mathbf{r}_t$. In particular, at each time-slot $t$, the algorithm generates $\boldsymbol{\gamma}_t$
from a multivariate uniform distribution with uncorrelated components, constrained within the range $[0, \eta]^N$,
%  from a multivariate uniform distribution in $[0, \eta]^N$,
and it updates the decision vector with the minimizer of $\scalar{\mathbf{x}}{\mathbf{\hat r}_{1:t-1} +  \boldsymbol{\gamma}_t}$ over $\mathbf{x} \in \mathcal{X}$.

%Once the estimation is observed, the algorithm updates the cumulative cost. %with the estimation $\mathbf{\hat r}_t$. 
%We want to highlight that NFPL is not specific to the caching problem but it can deal with any general online learning problem. More specifically, the set of the decisions $\mathcal{X}$
%Our proposed algorithm $1$, we call it Noisy Follow the Perturbed Leader (NFPL),  follows the same procedure as FPL with uniform noise but using at each time step, the estimation $\hat r_t$ instead of the real cost vector $r_t$. Algorithm $1$ is not specific to the caching problem but more general to any online learning problem. More specifically, the set of decisions $\mathcal{X}$ could be any other compact set with $l_1$ diameter $D = \sup_{x,y \in \mathcal{X}} \norm{x-y}_{1}$. The set $\bar{\mathcal{B}}$ of costs could be any other with bounded $l_1$ norm for every one of its elements, 

The performance of NFPL in terms of regret, as defined in~\eqref{eq:pseudoregret}, is expressed by the following theorem. 
\begin{theorem}[Regret bound NFPL]
% For $\eta = \sqrt{\frac{\hat R\cdot \hat A \cdot T}{D}}$,
NFPL has the following regret bound:
% the regret of NFPL verifies: 
        \begin{align} \label{e:NFPL-regret-bound}
                \nonumber \bar{\mathcal{R}}_{T}(\text{NFPL}) \leq 2 \sqrt{\hat R\cdot \hat A \cdot D\cdot T} \ . 
        \end{align}
\end{theorem}

\begin{IEEEproof}
Let $\{\mathbf{r}_t\}_{1}^{T}$ be a sequence of requests vectors, $\{\mathbf{\hat r}_t\}_{1}^{T}$ a realization from $\{\mathbf{r}_t\}_{1}^{T}$'s unbiased estimator and $\{\boldsymbol{\gamma}_t\}_{1}^{T}$ realizations from a multivariate uniform distribution with uncorrelated components, constrained within the range $[0, \eta]^N$. 
   The cost of NFPL given $\{\mathbf{r}_t, \mathbf{\hat r}_t , \boldsymbol{\gamma}_t\}_{1}^{T}$ is expressed as: 
    \begin{align}
        \text{NFPL}_{T} = \sum_{t=1}^{T} \scalar{\mathbf{r}_t}{ M(\mathbf{\hat r}_{1:t-1} + \boldsymbol{\gamma}_t)}\ .
    \end{align}
It is convenient to define the following two quantities: 
\begin{align}
  &\hatname{NFPL}_{T} = \sum_{t=1}^{T} \scalar{\mathbf{\hat r}_t} {M(\mathbf{\hat r}_{1:t-1} + \boldsymbol{\gamma}_t)}\ ,\\
  &\hatname{OPT}_{T} = \scalar{\mathbf{\hat r}_{1:T}}{M(\mathbf{\hat r}_{1:T})}\ . 
 \end{align}
% We similarly define the policy $\hat{\text{NFPL}}$ that at each time step $t$, chooses the sames state as NFPL $M(\hat r_{0:t-1})$, but its cost is evaluated with respect to the noisy cost vectors $\har r_t$, more specifically its cost is given by: 
% \begin{align}
%   \hatname{NFPL}_{T} = \sum_{t=1}^{T} \scalar{\hat r_t} {M(\hat r_{0:t-1})}   \ . 
% \end{align}
% We also define $\hat{\text{OPT}}$, the minimum cost incurred under the sequence $\{\hat{r_t}\}_{0}^{T}$ expressed as: 
% \begin{align}
%     \hat{\text{OPT}}_{T} = \scalar{\hat r_{1:T}}{M(\hat r_{1:T})}\ . 
% \end{align}
We compute the expectation, by considering the randomness of $\{\mathbf{\hat r}_t , \boldsymbol{\gamma}_t\}_{1}^{T}$, of the difference between the cost of NFPL and $\text{OPT}_{T}= \scalar{\mathbf{r}_{1:T}}{M(\mathbf{r}_{1:T})}$ as follows:
%G: this is wrong (I had already written it on the pages I gave to Younes), the supremum is missing. You need to say that you do the calculation for a specific sequence r_t and then take the expectation
%Y: True it is not clear, I'm modifying it. 

\begin{align} \nonumber
 &\E{\text{NFPL}_{T} - \text{OPT}_{T}} \\  \nonumber
&= \E{\text{NFPL}_{T} - \hatname{NFPL}_{T}}  + \E{\hatname{NFPL}_{T} - \hatname{OPT}_{T}}\\ \label{e:proof-NFPL4}
&\quad + \E{ \hatname{OPT}_{T} -\text{OPT}_{T}} \ .
\end{align}
We have: 
\begin{align} \label{e:proof-NFPL1}
    &\E{\text{NFPL}_{T} - \hatname{NFPL}_{T}} =0\ ,\\ \label{e:proof-NFPL2}
    &\E{\hatname{OPT}_{T}-\text{OPT}_{T}} \leq 0 \ ,\\ 
    \label{e:proof-NFPL3}
    &\E{\hatname{NFPL}_{T} - \hatname{OPT}_{T}} \leq 2\sqrt{\hat R\cdot \hat A\cdot D\cdot T } \ .
\end{align}
The random vectors $\mathbf{\hat {r}}_t$ and $M(\mathbf{\hat {r}}_{1:t-1} +\boldsymbol{\gamma}_t)$ are independent, hence $\E{\scalar{\mathbf{\hat r}_t}{M(\mathbf{\hat r}_{1:t-1} + \boldsymbol{\gamma}_t)} } = \scalar{\mathbf{r}_t}{\E{M(\mathbf{\hat r}_{1:t-1}+\boldsymbol{\gamma}_t)}}$ and by linearity of the expectation we deduce \eqref{e:proof-NFPL1}. 
% The equality \eqref{e:proof-NFPL1} follows from the estimations of the noisy cost at each time step being independent, then in particular $\hat r_t$ and $\hat r_{0:t-1}$ are independent and thus $\E{\scalar{\hat r_t}{M(\hat r_{0:t-1})} } = \scalar{r_t}{M(\hat r_{0:t-1})}$.
We have that $\hatname{OPT}\leq \scalar{\mathbf{\hat r}_{1:T}}{M(\mathbf{r}_{1:T})} $, we get then \eqref{e:proof-NFPL2}.  
% The inequality \eqref{e:proof-NFPL2} is because $\hatname{OPT}\leq \hat r_{1:T} M(r_{1:T}) $.
The quantity $\hatname{NFPL}_{T} - \hatname{OPT}_{T}$ can be seen as the difference between the cost of an FPL algorithm with uniform noise, that observes costs $\{\mathbf{\hat{r}}_t\}_{1}^{T}$, minus the cost incurred by the optimal static allocation $x^{*} = M(\mathbf{\hat r}_{1:T})$. Therefore, applying \cite[Theorem 1.1 a)]{kalai2005efficient} with $\epsilon = 1/\eta$ such that $\eta = \sqrt{\hat R\cdot \hat A \cdot T/D}$, we get:
\begin{equation*}
\Ex{\hat{\text{NFPL}}_{T} - \hat{\text{OPT}}_{T}}{\{\boldsymbol{\gamma}_t\}_{1}^{T}} \leq 2\sqrt{\hat R \cdot \hat A \cdot D \cdot T} 
\end{equation*}
for any $\{\mathbf{\hat r}_t\}_{1}^{T}$, and by taking the expectation over the randomness of $\{\mathbf{\hat r}_t\}_{1}^{T}$ in both sides of the last inequality, we find \eqref{e:proof-NFPL3}. Plugging \eqref{e:proof-NFPL1}, \eqref{e:proof-NFPL2} and \eqref{e:proof-NFPL3} in \eqref{e:proof-NFPL4}, we deduce that $\E{\text{NFPL}_{T} - \text{OPT}_{T}}\leq 2\sqrt{\hat R\cdot \hat A\cdot D\cdot T}$ for every $\{\mathbf{r}_t\}_{1}^{T}$,  concluding the proof. 
%
% We deduce then that $\E{\text{NFPL}_{T} - \text{OPT}_{T}} \leq 2\sqrt{\hat R\cdot \hat A\cdot D} \times \sqrt{T}$, since the bound is independent from the $\{r_t\}_{1}^{T}$ we find the desired result. 
\end{IEEEproof}

\begin{remark}
The bound on NFPL's regret in Theorem 1 can be written as: $\alpha \cdot \beta$ where $\alpha = \hat R \cdot \hat A / (R \cdot A) $, $\beta = 2\sqrt{R\cdot A \cdot D\cdot T}$, $R=\sup_{\mathbf{x}\in \mathcal{X}, \mathbf{r} \in \mathcal{\bar B}} \scalar{\mathbf{r}}{\mathbf{x}} $ and $A = \sup_{\mathbf{r}\in \mathcal{\bar B}} \norm{\mathbf{r}}_1$. Observe that $\beta$ is FPL's classical regret bound presented in \cite[Theorem 1.1 a)]{kalai2005efficient}. Moreover, it is easy to verify that $\alpha$ is greater than or equal to 1, representing a constant that captures the effect of the utilization of noisy costs in the regret bound.


% It is easy to check that $\alpha \geq 1$, which is a constant capturing the trade-off between the regret bound and the use of noisy costs.   



% FPL algorithm for online linear learning as presented in \cite{kalai2005efficient} has a regret
%G: is this expected regret or pseudo-regret? the relation with what is discussed here it unclear. is kalai2005efficient about FPL with known costs? If so, we should not say that we do worse as our constants boil down to theirs and we recover their result.
%Y: Yes I agree 
% bound of $2\cdot \sqrt{R\cdot A \cdot D\cdot T}$ where $R =\sup_{x\in \mathcal{X}, r \in \mathcal{B}} \scalar{r}{x} $ and $A = \sup_{r\in \mathcal{B}} \norm{r}_1$. When the costs vectors estimations are accurate, i.e. $\hat r_t = r_t$, we recover the bounds for FPL with uniform noise in \cite[Theorem 1.1 a)]{kalai2005efficient}. 
%G: the definition of A is incomplete
%Y: Done 

% It is easy to check that $\hat A\geq A$ and $\hat R \geq R$. It follows that the bound for FPL would be tighter than the one we proved. The trade-off is expressed by the ratio $\sqrt{\frac{\hat R \cdot \hat A }{R \cdot A}}$. 
\end{remark}

%Y: I think it is a good idea to say that from now on we only talk about the caching setting and specify the section II again, as Giovanni did in the beginning of Section III
We now study three specific cases of the unbiased estimator in the online caching setting: i) $\mathbf{\hat r}_t = \mathbf{r}_t$, i.e., the estimator is deterministic and always correct in Section~\ref{ss:FPL-caching}; 
ii) the case where a fixed number of requests is sampled within each batch and  iii) the case where each request is sampled with a given probability in Section~\ref{ss:NFPL-Caching-Fixed}. 



\begin{figure*}[t]
    \begin{subfigure}{0.32\linewidth}
  \centering
  \includegraphics[width=0.99\linewidth]{FIGURES/NACRoundRobinK100B200M50.pdf}
\caption{$C=100$}
\label{fig:NACRRSmall}
\end{subfigure}
\hfill
\begin{subfigure}{0.32\linewidth}
  \centering
  \includegraphics[width=0.99\linewidth, keepaspectratio]{FIGURES/NACRoundRobinK200B200M50.pdf}
  \caption{$C=200$}
  \label{fig:hit-rate-d2}
\end{subfigure}
\hfill
 \begin{subfigure}{0.32\linewidth}
      \centering  
    \includegraphics[width=0.99\linewidth,keepaspectratio]{FIGURES/NACRoundRobinK500B200M50.pdf}
    \caption{$C=500$}
    \label{fig:hit-rate-amazon}
\end{subfigure}
    \caption{Average miss ratio in the round-robin trace, $N=10^{4}$, $B=200$, $50$ runs.}
    \label{fig:hit-rates} 
    \vspace{-0.1in}
\end{figure*}

\subsection{FPL for Caching}
\label{ss:FPL-caching}
In the online caching problem, the case where $\mathbf{\hat r}_t = \mathbf{r}_t$ translates in dealing with the exact file requests. The following result applies to the online caching problem with batched requests. 
%We consider a particular case to adapt Algorithm~\ref{alg:NFPL} for the batched caching problem. The decisions set and the costs set will be as defined in Section~\ref{sec:bacground}. Moreover, we consider the deterministic case where the estimator $\hat{\mathbf{r_{t}}}$ is always exact, i.e. $\hat{\mathbf{r}_t} = \mathbf{r}_t$. We deduce then the following result: 
\begin{corollary} [Regret bound FPL caching] \label{co:FPL-uniform-noise}
Algorithm 1 applied for online caching with exact requests has the following regret bound: 
\begin{align}
           \bar{\mathcal{R}}_{T}(\text{FPL})
& \leq 2\sqrt{2}\cdot B \sqrt{C \cdot T}\ .
\end{align}
\end{corollary}
\begin{IEEEproof}
%Y: Sometimes We talk about Caching, some others about Online Caching. 
We utilize Theorem 1 to address the online caching problem with $\mathbf{\hat r}_t = \mathbf{r}_t$. As a consequence, we have $D\leq 2\cdot C$, $\hat R = \hat A = B$, allowing us to obtain the desired result.
%
% We apply Theorem $1$ for the case where the decision set $\mathcal{X}$ is as in \eqref{eq:Capped-Simplex}, implying that the diameter $D$ is equal to $2\cdot C$.
%G: isn't this always true also when C > N/2?
%Y: Yes, True the diameter might be smaller, but it is still an upper bound. 
% Also, the costs set $\bar{\mathcal{B}}$ is as in \eqref{eq:requests_set} and the unbiased estimator $\hat {\mathbf{r}_t}$ is always equal to the request $\mathbf{r}_t$. It follows that  $\mathcal{\bar{B}}= \hat{\mathcal{B}}$ and then, by definition of $\mathcal{\bar{B}}$, it follows that $\hat A=B$ and $\hat R=B$. Replacing the constants $\hat R, \hat A$ and $D$ in the result of Theorem $1$ we get our result. 
\end{IEEEproof}

In~\cite{bhattacharjee2020fundamental} Bhattacharjee et al. proposed an FPL-based algorithm with a Gaussian noise for the online caching problem and derived a bound on the regret (according to the regret definition~\eqref{eq:regret}). The result is copied next for completeness. 

\begin{theorem}\cite[Thm. 3]{bhattacharjee2020fundamental}
\label{th:FPL-gaussian-noise}
FPL applied to online caching with noise vectors $\{\boldsymbol{\gamma}_t\}_{1}^{T}$, where $\boldsymbol{\gamma}_t/\eta$ is drawn from a standard multivariate normal distribution, has the following expected regret bound:


%   For $\eta = \frac{1}{4\pi (\ln N)^{1/4}} \cdot \sqrt{\frac{T}{C}}$ and for $\gamma_t/\eta$ drawn standard multivariate normal distribution,  the expected regret of FPL is given by: 
  \begin{align}
      \mathcal{R}_{T}(\text{FPL})  \leq 1.51 \cdot (\ln N)^{1/4} \cdot \sqrt{C\cdot T}\ .
  \end{align}
\end{theorem}

Since $\mathcal{\bar R}_T \leq \mathcal{R}_T$, the regret bound is also valid for the weak regret defined in~\eqref{eq:pseudoregret}. In this view, our analysis presents two main novelties. First, our bound in Corollary~\ref{co:FPL-uniform-noise} is also valid in the case where the requests are batched, which is of practical interest since updating the cache at each request might be computationally impractical due to the high request rate. Second, even when the batch size $B$ is equal to 1, we provide a bound that does not depend on the catalogue size, and hence it will not diverge as $N$ goes to infinity. %Our analysis has advantage over state of the art FPL algorithm for caching in two dimensions. First, our bounds are also valid when requests are batched, which is of practical interest, since updating the cache at each time step might be unfeasible due to the high request rate. Second, even for the case when the batch size $B=1$, our regret bounds are tighter for a catalogue size $N\geq 13$. Moreover, \cite{bhattacharjee2020fundamental} bounds diverge as $N$ goes to infinity in contrast with our bounds that are independent of the catalogue size.

\subsection{NFPL for Caching}
\label{ss:NFPL-Caching-Fixed}
In the caching problem, especially in cases where the request rate is very high~\cite{estan2002new}, the sample of the actual requests within each batch can allow the use of slower and cheaper memory. In what follows we take into account two different ways of sampling requests inside each batch of requests. First, we consider the case where the caching system samples a fixed number of requests from each batch. Second, we consider the case where each request of the batch is independently sampled with a specified probability.

{\noindent \textbf{Fixed number of samples}}. 
%For the caching problem, it is of interest to consider only a subset of requests at each batch of size $l<B$. This is beneficial as the rate by which counters are updated is smaller and hence it can be afforded to use a slower cheaper memory for storing counts for each object. 
%We consider then the setting where we have access a sample $l$ out of $B$ requests, chosen uniformly at random from the batch. If $s_t$ is the sequence of requests in the batch, with frequency count for each object inside the batch $r_t$, $\hat s_t$ is sub-sequence of $s_t$ with length $l<B$ and $\hat d_t$ is the frequency count for each object inside the batch $\hat s_t$ . The unbiased estimator in this case is given by: 
We study the setting where the caching system has access to a sample of $b < B$
%G: "b" instead of "l"?
requests uniformly chosen at random from the batch at each time-slot. Let $\mathbf{\hat d}_t$ denote the vector of requests for each file in the sampled batch. We then use the following unbiased estimator for $\mathbf{r}_t$:
\begin{equation}\label{e:fixed-batch}
        \mathbf{\hat{r}}_t  =   \frac{B}{b} \cdot  \mathbf{\hat{d}}_t: \; \E{\mathbf{\hat r}_t} = \mathbf{r}_t\ .
\end{equation}
The performance of NFPL in terms of regret, for online caching with noisy requests as in \eqref{e:fixed-batch},  is expressed in the following corollary. 
% Using NFPL in this setting, we obtain the following bound:
\begin{corollary}[Regret bound NFPL with fixed sub-batch size]\label{co:NFPL-caching-fixed-subBatch}
      Algorithm 1 applied for caching with noisy requests estimates as in \eqref{e:fixed-batch}, has the following regret bound: 
        \begin{align}
                 \bar{\mathcal{R}}_{T}(\text{NFPL}) \leq 2\sqrt{2} \cdot B \sqrt{C\cdot T}\ . 
        \end{align}
\end{corollary}
\begin{IEEEproof}
We utilize Theorem 1 in the context of the online caching setting. Consequently, we establish that $D\leq 2\cdot C$. Considering the request vectors estimator given by equation \eqref{e:fixed-batch}, it can be observed that for every realization of $\mathbf{\hat r}_t$, its $l_1$ norm is equal to the batch size $B$. Therefore, we have ~$\hat A= \hat R = B$, which concludes the proof.
        % We apply Theorem $1$ for the case where $\mathcal{X}$ is as in \eqref{eq:Capped-Simplex}, implying that the diameter $D$ is equal to $2\cdot C$. The costs set $\bar{\mathcal{B}}$ is as in \eqref{eq:requests_set} and the unbiased estimator $\hat {\mathbf{r}_t}$ is given in \eqref{e:fixed-batch}. Notice that in this case $\norm{\hat{\mathbf{r}_t}}_1 = B$ for every realization we deduce then that $\hat A = B$ and $\hat R = B$. Replacing the constants $\hat R, \hat A$ and $D$ in the result of Theorem $1$ we get our result. 
\end{IEEEproof}
\begin{remark}
The NFPL (Noisy-Follow-the-Perturbed-Leader) algorithm, when used with the unbiased estimator described in \eqref{e:fixed-batch} for the request vectors $\mathbf{r}_t$, provides the same regret guarantees as if the request vectors were exact (See Corollary~\ref{co:FPL-uniform-noise}). However, it is worth noting that in Section~\ref{sec:experiments}, we show that using small values of $b$ can decrease the performance of the algorithm. 



% The regret bound in Corollary \ref{co:NFPL-caching-fixed-subBatch} is independent from the sub-batch size $b$. However, we will show in Section~\ref{sec:experiments} that the smaller is the value of $b$, the higher is the variability in the cost of our algorithm.  
\end{remark}


{\noindent \textbf{Variable number of samples}}. Another approach is to consider a sub-batch where each request is independently sampled with probability $f>0$ at each iteration. In this case, the size of the sub-batch is a random variable and we consider the following unbiased estimator:
%Another model, is to consider a sub-batch that samples each request with a probability $f>0$ at each time step, in this case the size of the batch is a random variable and the unbiased estimator $\hat r_t$ is expressed in this case as: 
\begin{equation}\label{e:estimator-rt-f}
    \mathbf{\hat r}_t = \frac{1}{f} \cdot \mathbf{\hat d}_t: \; \E{\mathbf{\hat r}_t} = \mathbf{r}_t\ , 
\end{equation}
where $\mathbf{\hat d}_t$ is defined as in \eqref{e:fixed-batch}. The performance of NFPL in terms of regret, for online caching with noisy requests as in \eqref{e:estimator-rt-f}, is expressed in the following corollary. 

% In this case, NFPL achieves the following regret bound:
\begin{corollary}[Regret bound NFPL with variable sub-batch size]\label{c:sampling}
      Algorithm 1 applied for caching with noisy requests estimates as in \eqref{e:estimator-rt-f}, has the following regret bound: 
        \begin{align}
                 \mathcal{\bar{R}}_{T}(\text{NFPL}) \leq 2\sqrt{2} \cdot \frac{B}{f} \cdot \sqrt{C\cdot T} \ . 
        \end{align}
\end{corollary}
\begin{IEEEproof}
We apply Theorem 1 to the online caching setting, leading us to establish that $D$ is bounded by $2\cdot C$. Examining the request vectors estimator described in equation \eqref{e:estimator-rt-f}, we observe that the maximum of $\norm{\mathbf{\hat r}_t}_1$ is attained when the sub-batch includes all the requests from the batch. As a result, we have $\hat A = \hat R = B/f$, which concludes the proof. 
\end{IEEEproof}


\begin{remark}
Indeed, it holds true that even when considering extremely small values for $f$, which represents the sampling probability, Corollary \ref{c:sampling} demonstrates that sublinear regret is still achieved. However, if the time horizon is not sufficiently large, the bounds provided in Corollary \ref{c:sampling} lose their significance. This is because, in the caching problem, $\mathcal{\bar{R}}_T(\mathcal{A})$ is always smaller than $B\cdot T$ for any caching policy $\mathcal{A}$. 
\end{remark}

%Y: The remark we can say in this section is that all these algorithms has \mathcal{O}(\sqrt{T}) regret despite the noisy requests. 
 


% \begin{remark}
% Building on Remark $1$, $\alpha = 1/f$. Notice that for $f= \frac{l}{B}$, on expectation the number of requests in the sub-batch is the same as when using the estimator in \eqref{e:fixed-batch}. But the bound for the latter is tighter
%  % With comparison to the regret bound for the exact requests case, Corollary 3 regret bound is 
%     % The bound in Corollary~\ref{c:sampling} shows the dependency on the sampling probability $f$. Surprisingly, we always have $\bar{\mathcal{R}}_{T} = \mathcal{O}(\sqrt{T})$ but as $f$ goes to $0$, the constant in our bound for the regret becomes larger.  
% \end{remark}
%FF: we should comment more here.


==> Old_background.tex <==
We consider a single-cache system in which file requests for a catalogue with $N$ files can either be served locally by a cache with finite capacity $C$ or, in the case of a file miss, by a remote server. 
%The latter scenario incurs a file-dependent cost associated with retrieving the file. This cost may represent the time needed to fetch the file from the remote server or a monetary expense due to the use of network infrastructure.
%G: WHY TALK ABOUT FILE-DEPENDENT COSTS IF LATER WE JUST LOOK AT THE MISS COST.

{\noindent \bf Cache state}. The local cache has a capacity $C \in \{1,\ldots,N\}$ and stores files in their entirety. The cache state at time $t$ is represented by the vector $\mathbf{x}_t = [x_{t,i}]_{i\in \mathcal{N}}$, which indicates the files missing in the cache; that is, $x_{t,i} = 1$ if and only if file $i$ is not stored in the cache at time $t$. A feasible cache allocation is then represented by a vector in the set:

\begin{equation}\label{eq:Capped-Simplex}
\mathcal{X} = \left \{ \mathbf{x} \in \{0,1\}^{N} \Bigg| \sum_{i=1}^N x_{i} = N-C \right \}.
\end{equation}

%The set $\mathcal{X}$ represents the capped simplex defined by the capacity constraint of the local cache.
%G: technically this is not the capped-simplex


{\noindent \bf Cache updates}. Although caching policies are often assumed to update their state after each request, in high request regimes or when cache updates are computationally or communicationally expensive, the cache may update its state after receiving a batch of $B$ requests~\cite{salem2021no}.
We study caching policies in this more general setting and consider a time-slotted operation. At each time-slot $t=1,\ldots,T$,
$B$ requests are collected from the users and the cache state is updated. The request process is represented as a sequence of vectors $\mathbf{r}_t = (r_{t,i} \in \mathbb{N}: i \in \mathcal{N})$ $\forall t$, where $r_{t,i}$ is the number of requests received for file $i$ at time $t$ in a file batch of size $B$. All the requests belong to the set
\begin{equation}\label{eq:requests_set}
%G: why this bar?
\bar{\mathcal{B}} = \left \{ \mathbf{r}_t \in \mathbb{N}^N, t = 1, \dots, T \Bigg| \sum_{i=1}^N r_{t,i} = B \right \}.
\end{equation}
%Maybe here we could introduce the notation for norm 1
{\noindent \bf Cost}. At each time-slot $t$, the caching system pays a cost equal to the number file misses, i.e., the number of files that must be retrieved by the remote server. Formally:
\begin{equation}\label{eq:cost}
\phi_{\mathbf{r}_t}(\mathbf{x}_t) = \scalar{\mathbf{r}_t}{\mathbf{x}_t}= \sum_{i=1}^N r_{t,i} x_{t,i}\ ,
\end{equation}
where $\scalar{\mathbf{r}}{\mathbf{x}} \triangleq \sum_{i=1}^N r_{i} x_i$ denotes the scalar product of the two vectors $\mathbf{r}$ and $\mathbf{x}$.
% We have that: 
% \begin{align}
%     R &= \sup_{\mathbf{x},\mathbf{y}\in \mathcal{X}, t \in [T]} |\scalar{\mathbf{r}_t}{(\mathbf{x}-\mathbf{y})}| \leq B \cdot D_2 = \sqrt{2C}\cdot B \ .
% \end{align}
%Do we really need to define R ? 

For the sake of conciseness, we introduce the following  notation. For any vector $\mathbf{r}$, we denote by $M(\mathbf{r})$ an arbitrary element of $\arg\min_{\mathbf{x}\in \mathcal{X}} \scalar{\mathbf{r}}{\mathbf{x}}$. Furthermore, given a sequence of vectors $(\mathbf{r}_1, \dots, \mathbf{r}_t)$, we represent their aggregate sum as $\mathbf{r}_{1:t}\triangleq \sum_{s=1}^t \mathbf{r}_s$.

\subsection{Online Caching}
%G: NO, THIS IS NOT TECHNICALLY CONVEX OPTIMIZATION, BECAUSE THE VARIABLE IS DISCRETE
Caching  may be framed as an online learning problem~\cite{hazan2016introduction}, where an agent (the caching system) chooses an action $\mathbf{x}_t$ from a set $\mathcal{X}$ at each time-slot~$t$ before an adversary selects the cost function $\phi_{\mathbf{r}_t}: \mathcal X \to \mathbb R$.
%, i.e., the system changes the cache state before experiencing the cost. 
%Y: The adversary only reveals the cost $r_t$, but the function depends on the player decision. Kalai and Vempla Paper has a linear model that fits the caching problem. Is citing hazan the right thing here ? 

The cache state is determined by an online algorithm $\mathcal{A}$ that, at each time-slot $t$, computes the cache state $\mathbf{x}_{t+1}$ for the next time-slot given the current state $\mathbf{x}_t$ and the cost functions incurred so far, which, in our application, are  determined solely by the sequence of requests up to time~$t$, that is $\{\mathbf{r_{s}}\}_{s=1}^{t}$. 

The main performance metric used to evaluate an online algorithm $\mathcal{A}$ is the regret, for which two different definitions are available in case of randomness in the algorithm. The expected regret is defined as 

\begin{equation}\label{eq:regret}
    \mathcal{R}_T(\mathcal A) = \E{\sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{\sum_{t=1}^{T} \scalar{\mathbf{r}_t}{\mathbf{x}_t} - \text{OPT}_T\right \}},
\end{equation}
where $\text{OPT}_T = \scalar{\mathbf{r}_{1:T}}{M(\mathbf{r}_{1:T})}$ is the
%Y: We do not need to say the minimum
% minimum
cost incurred under the request sequence $\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}$ by the optimal static allocation $\mathbf{x}^* = M(\mathbf{r}_{1:T})$, and the expectation is taken over any random choice of the algorithm $\mathcal A$.
The expected regret quantifies then the performance gap over a time horizon $T$ between the algorithm $\mathcal{A}$ and the best static cache allocation with hindsight.
%decision $\mathbf{x}^*$ in hindsight for any sequence of requests, i.e., $\mathbf{x}^* = \arg\min_{\mathbf{x} \in \mathcal{X}} \sum_{t=1}^T f_{\mathbf{r}_t}(\textbf{x})$. 
In contrast, the mean regret~\cite{belmega2018online} (also called pseudo-regret or weak regret) is defined as 
\begin{equation}\label{eq:pseudoregret}
    \bar{\mathcal{R}}_T(\mathcal A) = \sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_t\}} \left \{ \E{\sum_{t=1}^{T} \scalar{\mathbf{r}_t}{\mathbf{x}_t}} - \text{OPT}_T\right \}.
\end{equation}
The interpretation remains analogous, but the mean regret involves comparing the \emph{expected} performance of algorithm $\mathcal A$ with that of the optimal static cache allocation. Applying Jensen's inequality leads one directly to conclude that $\bar{\mathcal{R}}_T \le  \mathcal{R}_T$. Our findings are articulated in terms of the mean regret, which we will henceforth refer to as just 'regret'.

Due to the supremum over all request sequences in~\eqref{eq:regret} and in~\eqref{eq:pseudoregret}, regret metrics do not make any assumptions about the nature of the request sequence (e.g., no statistical regularity). This means that the request sequence could be generated by an adversary seeking to degrade the performance of the caching system.

In this setting, one aims for an algorithm with sublinear regret, $\bar{\mathcal{R}}_T(\mathcal{A}) = o(T)$. These algorithms are commonly known as no-regret algorithms since their time-average cost approaches the optimal static policy's cost as $T$ grows.

%G: WRITE SOMETHING ALONG THE FOLLOWING LINES:
%Online algorithms have regret can achieve a regret bound of at most $\sqrt{T}$~\cite{mcmahan2017survey}. 
%G: exactly the opposite, this is a lower bound for caching problem (cite sinha, it has the probabilistic method proof we discussed). I am not sure such result is in mcmahan, as it is not true for general online learning algorithm (bandit algorithm can have \log t). I do not have time to check this, also because I think such bounds are in terms of the expected regret rather than the mean regret.
Various algorithms, such as Online Gradient Descent (OGD) and Follow-the-Regularized-Leader (FTRL), can attain $\mathcal O(\sqrt{T})$-regret for caching problems~\cite{paschos2019learning,mhaisen2022online}. However, their cache update procedures necessitate projecting a tentative solution back onto the feasible set, which incurs $O(N^2)$ computational cost~\cite{wang2015projection}. %in the general case~\cite{wang2015projection} of batched requests~\cite{salem2021no}. %and $O(...)$ for OGD and FRL, respectively~\cite{wang2015projection,}. 
%G: check the projection cost in Tareq, I think it is smaller.
%F: for OGD, seen as a particular case of OMD, we can achieve O(N + ClogC) but for FTRL we should keep O(N^2).
In the next section, we present a lightweight caching algorithm with $\mathcal{O}(\sqrt{T})$-regret.% according to the regret definition in~\eqref{eq:pseudoregret}.

\subsection{Follow-the-Perturbed-Leader (FPL)}
Within the domain of online learning, the Follow-the-Perturbed-Leader (FPL) algorithm is a notable projection-free methodology known to achieve sublinear regret. This algorithm was initially introduced by Vempala et al.~\cite{kalai2005efficient}, and later studied within the caching framework by Bhattacharjee et al.~\cite{bhattacharjee2020fundamental}. 

The FPL algorithm serves as a refined version of the traditional Follow-the-Leader (FTL) algorithm~\cite{littlestone1994weighted}. The latter greedily selects the state that would have minimized the past cumulative cost, i.e., $\mathbf{x}_{t+1}(\text{FTL}) = M(\mathbf{r}_{1:t})$. 

While the FTL algorithm proves optimal when cost functions are sampled from a stationary distribution, it unfortunately yields linear regret in adversarial settings~\cite{de2014follow}.
%The behaviour of FTL can be easily exploited by an adversary by always requesting all the files that are not stored in the current time-slot leading to a linear regret for the algorithm.
%Younes: Here we are talking about online convex optimization in general so I think it is a bit weird to go back to caching. I think maybe we could just cite a paper that shows FTL is not good OK

%Younes: Maybe this is the right time To introduce the notation M(r_{i:j}) OK
FPL algorithm improves the performance of FTL by incorporating
% an artificial initial vector of requests, $\mathbf{r}_0$.
a noise vector $\boldsymbol{\gamma}_t$ at each time step $t$.
This vector's components are independent and identically distributed (i.i.d.) random variables, pulled from a distinct distribution (such as the uniform and exponential distributions in~\cite{kalai2005efficient}, and the Gaussian distribution in~\cite{bhattacharjee2020fundamental}). The update process unfolds similarly to FTL:

 \begin{equation}
    \label{e:fpl_update}
     \mathbf{x}_{t+1}(\text{FPL}) = M(\mathbf{r}_{1:t}+\boldsymbol{\gamma}_t) \ .
 \end{equation}
%As described in~\cite{bhattacharjee2020fundamental}, in the case of caching, the algorithm first samples a vector of random variables $\boldsymbol \eta$. Then, at every time-slot, it adds the random noise to 
%the current cumulative cost vector $\mathbf{r}_{0:t}$. Finally, the algorithm caches $C$ files with the lowest perturbed cumulative cost at each time-slot.
%G: I commented what above because it is a wrong description of what is already said in e:fpl_update.
As shown in~\cite{bhattacharjee2020fundamental}, FPL provides optimal regret guarantees for the discrete caching problem. Moreover, the cache update, as specified in equation~\eqref{e:fpl_update}, involves storing the files that correspond to the largest elements of the vector $\mathbf{r}_{1:t}+\boldsymbol{\gamma}_t$. FPL cache update necessitates then a sorting operation. This operation is computationally less demanding than the projection step required by the FRL or OGD algorithms~\cite{paschos2020online}.
%Younes: Maybe here, we can just give the definition 
%Younes: We can here refer directly to OGD 

==> Recovery_Files/analysis.tex <==
The proof employs similar techniques used in the original paper of FPL \cite{kalai2005efficient}. Which makes use of the virtual policy that considers costs up to time $t$ at time step $t$. 

\begin{align}
    \widehat{\text{NBPL}}(1:T) = \sum_{t=1}^{T} \hat r_t \cdot M(\hat r_{0:t}).
\end{align}
For convenience, we define $\hat{\text{NFPL}}$ as the policy that takes the same decision as NFPL but the cost is also evaluated with respect to the noisy costs $\hat r_t$. More specifically: 
    \begin{align}
        &\widehat{\text{NFPL}}(1:T) = \sum_{t=1}^{T} \hat r_t \cdot M(\hat r_{0:t-1}).
    \end{align}
\color{blue}
\begin{lemma} \label{lem:hat-NFPL-NFPL}
NFPL and $\widehat{\text{NFPL}}$ have the same expected cost. 

\begin{equation}
    \Ex{\text{NFPL}}{\{\hat r_s\}_{0}^{T}} =   \Ex{\widehat{\text{NFPL}}}{\{\hat r_s\}_{0}^{T}} .   
\end{equation}
\color{black}
\begin{proof}
The random vectors $\hat r_t$ and $M(\hat r_{0:t-1})$ are independent, by linearity of the expectation, the result follows. 
\end{proof}
\end{lemma}


\color{black}
% \begin{remark}
%     The previous lemma is not valid for NBPL because $\hat r_t$ and $M(\hat r_{0:t})$ are clearly dependent. 
% \end{remark}

% \begin{lemma}
% $\hat{\text{NBPL}}$ is not that far from the static optimum 
% \begin{align}
%     \Ex{\hat{\text{NBPL}}}{\{r_s\}_{0}^{T}} \leq \text{OPT}(1:T) + \Ex{\hat r_0 \cdot (M(\hat r_{1:T})  - M(\hat r_0))}{r_s}
% \end{align}
% \begin{proof}
% Make use of the fact that: 
%     \begin{align}
%         \sum_{t=0}^{T} y_t \cdot M(y_{0:t}) \leq y_{0:T} M(y_{0:T}) 
%     \end{align}
% for any vectors $y_t$, it is proven in \cite{kalai2005efficient}. 
% \end{proof}
% \end{lemma}



% \begin{lemma}

% \begin{align}
%     \Ex{\hat r_0 \cdot (M(\hat r_{1:T})  - M(\hat r_0))}{r_s} \leq \eta \cdot D_1 
% \end{align}
 
% \end{lemma}

\color{blue}
\begin{lemma}\label{lem:hatNBPL-OPT}
\begin{align}
    \Ex{\widehat{\text{NBPL}}}{\hat \{r_s\}_{0}^{T}} \leq \text{OPT}(1:T) + \eta \cdot D_1 .
\end{align}
\color{black}
\begin{proof}
Make use of the fact that: 
    \begin{align}
        \sum_{t=0}^{T} y_t \cdot M(y_{0:t}) \leq y_{0:T} M(y_{0:T}) 
    \end{align}
for any vectors $y_t$, it is proven in \cite{kalai2005efficient}. For $y_t= \hat r_t$ we get: 

\begin{align}
     \sum_{t=0}^{T} \hat r_t \cdot M(\hat r_{0:t})
     &\leq \hat r_{0:T} M(\hat r_{0:T}) \\
     & \leq \hat r_{0:T} M(\hat r_{1:T}) \\ 
     & = \hat M(\hat r_{1:T})( \hat  r_{1:T} + \hat r_{0}) .
\end{align}
It follows that: 
\begin{align}
 \widehat{\text{NBPL}} 
 &=    \sum_{t=1}^{T} \hat r_t \cdot M(\hat r_{0:t}) \\
&\leq \hat r_{1:T} \cdot M(\hat r_{1:T})    + \hat r_0 \left( M(\hat r_{1:T}) - M(\hat r_0)\right)  \\ 
&\leq \hat r_{1:T} \cdot M(r_{1:T})+ \hat r_0 \left( M(\hat r_{1:T}) - M(\hat r_0)\right).
\end{align}
Taking the expectation over $\{\hat r_s\}_{0}^{T}$ and using Lemma 6 in \cite{RobertNotes} we get the desired result.

\end{proof}
\end{lemma}
\color{black}
\color{blue}
\begin{lemma}\label{lem:shifted-uniform-coupling}
Let $X$ be random vector with probability distribution $p$ over $\mathds{R}^{N}$, where each component is a uniform distribution in $[a_i,b_i]$,   $a,b\in \mathds{R}^{N}\times \mathds{R}^{N}$,$b_i-a_i = 2\eta >0$,  and the realization of each component is independent from the others. Let $Y$ be random variable with the same probability distribution as $X+r$, we call it $q$, where $r\in \mathds{R}^{N}$ such that $a+r<b$. There exist a coupling between $X$ and $Y$, $Z=(X,Y)$ such that: 
\begin{equation}
    \Proba{X \neq Y} \leq \frac{\norm{r}_1}{2\eta} .
\end{equation}
\color{black}
\begin{proof}
 We consider 
 
 \begin{equation}
     Y = \begin{cases}
      X &\text{ if }   a + r \leq  X \leq b\\
      X+ b-a &\text{otherwise}.
    \end{cases}
 \end{equation}
It is easy to check that if $X$ has distribution $p$ then $Y$ with the construction above has also distribution $q$. Moreover, 

\begin{align}
    \Proba{X\neq Y} 
&= \Proba{\exists i \in [N]:\; a_i \leq X_i \leq a_i + r_i } \\
&\leq \sum_{i=1}^{N} \Proba{ a_i \leq X_i \leq a_i + r_i} \\ 
&=  \sum_{i=1}^{N} r_i \cdot \frac{1}{b_i-a_i} \\
&\leq \frac{\norm{r}_1}{2\eta}\ .
\end{align}
\end{proof}
\end{lemma}
\color{blue}

\begin{lemma}\label{lem:NFPL-NBPL}
For any realization of $\{ \hat r_s\}_{1}^{T}$
    \begin{align}
        \Ex{\widehat{\text{NFPL}}}{\{\hat r_s \}_{1}^{T}} \leq \Ex{\widehat{\text{NBPL}}}{\{\hat r_s \}_{1}^{T}} + R \cdot \frac{B}{p} \cdot \frac{T}{2 \eta} \ .
    \end{align}
\color{black}
    \begin{proof}
    Follows directly from \cite{RobertNotes} Corollary 4 and Lemma 5, by considering the costs vector to be $\{\hat r_s\}_{1}^{T}$ and noticing that $\norm{\hat r_t}_1 \leq \frac{B}{p}$. The only problem is that there is a mistake in the proof of Lemma 5. More details: 
    \begin{align}
        \Ex{\widehat{\text{NFPL}} - \widehat{\text{NBPL}}}{\hat r_0}
&= \sum_{t=1}^{T} \hat r_t \cdot \Ex{M(\hat r_{0:t-1}) -M(\hat r_{0:t}) }{\hat r_0}
    \end{align}
$\hat r_{0:t-1}$ is are  uniform distribution $\hat r_{0:t}$ has a distribution of $\hat{r_{0:t-1}} + r_t$. Using Lemma \ref{lem:shifted-uniform-coupling}, we can find two random vectors $y_1$ and $y_2$ with the same distribution as $\hat r_{0:t-1}$ and $\hat r_{0:t}$, respectively. Moreover we have:   

\begin{align}
     \Proba{y_1 \neq y_2} \leq \frac{B}{p} \cdot \frac{1}{2 \eta} ,
\end{align}

\begin{align}
    &\hat r_t\cdot \Ex{M(\hat r_{0:t-1}) -M(\hat r_{0:t}) }{\hat r_0}\nonumber\\
    &= \hat r_t\cdot \Ex{M(y_1)-M(y_2)}{(y_1,y_2)} \\\nonumber
    & =\hat r_t \cdot( \Ex{M(y_1)-M(y_2)\mid y_1 = y_2}{(y_1,y_2)} \mu (y_1=y_2) \\ 
    &\;\;\;+  \Ex{M(y_1)-M(y_2)\mid y_1 = y_2}{(y_1,y_2)} \mu (y_1\neq y_2) )\\
    & = \hat r_t \cdot \Ex{M(y_1)-M(y_2)\mid y_1 = y_2}{(y_1,y_2)} \mu (y_1\neq y_2) \\ 
    &\leq R \cdot \frac{B}{p}\cdot \frac{1}{2\eta} \ .
\end{align}
By taking the expectation over $\{\hat r_s \}_{1}^{T}$ and then summing from $t=1$ to $T$, we get the desired result.
\end{proof}
\end{lemma}


\begin{proof}[Theorem 3] 
Simply combining Lemmas \ref{lem:hat-NFPL-NFPL}, \ref{lem:hatNBPL-OPT}, \ref{lem:NFPL-NBPL}. 
\end{proof}
\color{black}

==> Recovery_Files/approach1.tex <==
\subsection{FPL with noisy costs}


\begin{algorithm}[h] 
\KwIn{Set of decisions $\mathcal{X}$; Time Horizon $T$; $R, \; A, \; D$}
\KwOut{Sequence of decisions: $\{x_t\}_{1}^{T}$}

$\eta \gets \sqrt{\frac{R\cdot A \cdot T}{D}}$ \\ 
$\hat{\textbf{costs}} \gets  0$ ,  \\ 
\For{round $t=1,2,...,T$}{
$\mathbf{x_t} \gets M(\hat{\textbf{costs}} +  \textbf{Unif}\left(\left[0, \eta\right], \mathbb{I}_{N\times N}\right))$ \\ 
Observe $\hat{\mathbf{r_t}}$ \\
$\hat{\textbf{costs}} \gets \hat{\textbf{costs}} + \hat{r_t}$
}
\label{alg:NFPL}
\caption{Noisy Follow the Perturbed Leader with Uniform Noise (NFPL)}
\end{algorithm}


Our main contribution is proposing a more general version of the FPL algorithm where we do not have necessarily access to the exact cost vector, $r_t$, but only to its estimation: $\hat r_t$. $\hat r_t$ is an unbiased estimator of $r_t$ with bounded $l_1$ norm for every realization, i.e. 

\begin{align}
   \E{\hat r_t} = r_t , \; \sup_{t\in [T],\; \omega \in \Omega} \norm{\hat r_t (\omega)}_1 \leq A  
\end{align}
and $\norm{x}_1 = \sum_{i=1}^{N} \|x_i\|$ 
Our proposed algorithm $1$, we call it Noisy Follow the Perturbed Leader (NFPL),  follows the same procedure as FPL with uniform noise but using at each time step, the estimation $\hat r_t$ instead of the real cost vector $r_t$. Algorithm $1$ is not specific to the caching problem but more general to any online learning problem. More specifically, the set of decisions $\mathcal{X}$ could be any other compact set with $l_1$ diameter $D = \sup_{x,y \in \mathcal{X}} \norm{x-y}_{1}$. The set $\bar{\mathcal{B}}$ of costs could be any other with bounded $l_1$ norm for every one of its elements, 

The operation $M(\textbf{costs})$ corresponds   

\begin{align}
    &R = \sup_{x\in \mathcal{X}, t\in [T]} \scalar{r_t}{x}\\
    &D= \sup_{x,y \in \mathcal{X}} \norm{x-y}_{1} \\ 
    &A = \sup_{r\in \bar{\mathcal{B}}} \norm{r}_{1} 
\end{align}
\begin{theorem}[Regret bounds NFPL]
For $\eta = \sqrt{\frac{R\cdot A \cdot T}{D_1}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \Ex{  \mathcal{R}_{T}(\text{NFPL}) }{\{\hat r_t\}_{0}^{T}}\leq 2 \sqrt{R\cdot A \cdot D\cdot T}
        \end{align}
    where the expectation is taken over the randomness of $\{\hat r_t\}_{0}^{T}$.
    


\end{theorem}

\begin{IEEEproof}
   The cost of NFPL is given by: 
    \begin{align}
        \text{NFPL}_{T} = \sum_{t=1}^{T} \scalar{r_t}{ M(\hat r_{0:t-1})}\ .
    \end{align}
We similarly define the policy $\hat{\text{NFPL}}$ that plays the same actions as NFPL for a given $\{\hat r_t\}_{0}^{T}$ but evaluated with respect to the noisy requests, instead of the actual requests, more specifically its cost is given by: 

\begin{align}
   \hatname{NFPL}_{T} = \sum_{t=1}^{T} \scalar{\hat r_t} {M(\hat r_{0:t-1})} , \hat{\text{OPT}}_{T} = \scalar{\hat r_{1:T}}{M(\hat r_{1:T})}  \ . 
\end{align}
the regret can be written as: 
\begin{align}
    &\E{\mathcal{R}_{T}(\text{NFPL})} \\
&= \E{\text{NFPL}_{T} - \text{OPT}_{T}} \\ 
&= \E{\text{NFPL}_{T} - \hatname{NFPL}_{T}} + \\
&\;  \E{\hatname{NFPL}_{T} - \hatname{OPT}_{T}} + \E{ \hatname{OPT}_{T} -\text{OPT}_{T}}
\end{align}
We have: 
\begin{align} \label{e:proof-NFPL1}
    &\E{\text{NFPL}_{T} - \hatname{NFPL}_{T}} =0\\ \label{e:proof-NFPL2}
    &\E{\hatname{OPT}_{T}-\text{OPT}_{T}} \leq 0 \\ \label{e:proof-NFPL3}
    &\E{\hatname{NFPL}_{T} - \hatname{OPT}_{T}} \leq 2\sqrt{R\cdot D\cdot A} \times \sqrt{T} 
\end{align}
The equality \eqref{e:proof-NFPL1} follows from the estimation of the noisy estimate at each time step being independent, then $\hat r_t$ and $\hat r_{0:t-1}$ are independent. The inequality \eqref{e:proof-NFPL2} is because $\hatname{OPT}\leq \hat r_{1:T} M(r_{1:T}) $. The inequality \eqref{e:proof-NFPL3} follows from \cite[Theorem 1.1]{kalai2005efficient}. 
\end{IEEEproof}







\subsection{FPL for caching with exact requests}
We deduce the following corollary as a particular deterministic estimator, the real cost vector $r_t$.  

\begin{corollary} [Regret bounds FPL caching] \label{th:FPL-uniform-noise}
For $~\eta= B \sqrt{\frac{T}{2C}}$, FPL with uniform noise applied to caching has the following regret bounds
\begin{align}
          \E{  \mathcal{R}_{T}(\text{FPL}) }
& \leq 2\sqrt{2}\cdot  B \cdot \sqrt{C \cdot T}\ .
\end{align}
\end{corollary}
\begin{IEEEproof}
It is easy to show that the $l_1$ diameter of $\mathcal{X}$ $D_1 = 2\cdot C$ and the $l_2$ diameter is given by $D_2 = \sqrt{2\cdot C}.$, The batch size is fixed hence $\norm{r_t}_{1}=B$ and $ \norm{r_t}_2 \leq B$.  $ R = \sup_{t,x} r_t x$ then $R\leq B$. Then by applying Theorem (X) from \cite{kalai2005efficient} we get our result. 
\end{IEEEproof}
For the problem of caching, \cite{bhattacharjee2020fundamental} proposes FPL algorithm for caching with a Gaussian Noise. They prove the following regret bound. 

\begin{theorem}\cite[Theorem 3]{bhattacharjee2020fundamental}
\label{th:FPL-gaussian-noise}
  For $\eta = \frac{1}{4\pi (\ln N)^{1/4}} \cdot \sqrt{\frac{T}{C}}$ and for $\gamma_t$ normal gaussians. $r_0 = \eta \cdot \gamma_t$. The expected regret of FPL is given by: 
  \begin{align}
      \E{  \mathcal{R}_{T}(\text{FPL}) } \leq 1.51 \cdot (\ln N)^{1/4} \cdot \sqrt{C\cdot T}\ .
  \end{align}
\end{theorem}

Our analysis has advantage over state of the art FPL algorithm for caching in two dimensions. First, our bounds are also valid when requests are batched, which is of practical interest, since updating the cache at each time step might be unfeasible due to the high request rate. Second, even for the case when the batch size $B=1$, our regret bounds are tighter for a catalogue size $N\geq 13$. Moreover, \cite{bhattacharjee2020fundamental} bounds diverge as $N$ goes to infinity in contrast with our bounds that are independent of the catalogue size.


















\subsection{FPL for caching with noisy requests estimates}
For the caching problem, it is of interest to consider only a subset of requests at each batch of size $l<B$. This is beneficial as the rate by which counters are updated is smaller and hence it can be afforded to use a slower cheaper memory for storing counts for each object. We consider then the setting where we have access a sample $l$ out of $B$ requests, chosen uniformly at random from the batch. If $s_t$ is the sequence of requests in the batch, with frequency count for each object inside the batch $r_t$, $\hat s_t$ is sub-sequence of $s_t$ with length $l<B$ and $\hat d_t$ is the frequency count for each object inside the batch $\hat s_t$ . The unbiased estimator in this case is given by:         

\begin{equation}\label{e:fixed-batch}
    \hat r_t  =   \frac{B}{l} \cdot \hat d_t: \; \E{\hat r_t} = r_t, \; \sup_{t\in [T],\; \omega \in \Omega} \norm{\hat r_t(w)}_{1} = B
\end{equation}



    

\begin{corollary}[Regret Bounds NFPL with fixed size sub-batch]\label{co:NFPL-caching-fixed-subBatch}
      For $\eta = B \cdot \sqrt{\frac{T}{2\cdot C}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \E{  \mathcal{R}_{T}(\text{NFPL}) }\leq 2\sqrt{2} \cdot B \cdot \sqrt{C\cdot T}
        \end{align}
\end{corollary}

Another model, is to consider a sub-batch that samples each request with a probability $f>0$ at each time step, in this case the size of the batch is a random variable and the unbiased estimator $\hat r_t$ is expressed in this case as: 

\begin{equation}
    \hat r_t = \frac{1}{p} \cdot \hat d_t 
\end{equation}


\begin{corollary}[Regret Bounds NFPL sampling probability $f$]
      For $\eta = B \cdot \sqrt{\frac{T}{2\cdot C}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \E{  \mathcal{R}_{T}(\text{NFPL}) }\leq 2\sqrt{2} \cdot \frac{B}{f} \cdot \sqrt{C\cdot T}
        \end{align}
        
    \begin{IEEEproof}
        The proof follows from Theorem $1$ and noticing that $\norm{\hat r_t} \leq \frac{B}{f}$  
    \end{IEEEproof}
\end{corollary}

\begin{remark}
It is possible to prove the tighter bound without dependency on $f$ but I think it will require refering to results inside the notes of Kleinberg, maybe it is not worth it ? 
\end{remark}


% \begin{remark}
%  It seems that the difference between NFPL and FPL is the constant in the regret $\frac{1}{p}$. But NFPL has more variance, since the expectation is taken now over more randomness. 
% \end{remark}



% \begin{algorithm}[h] 
% \KwIn{$R,\; T,\; B, \; D_1$}
% \KwOut{Sequence of cached items: $\{x_t\}_{1}^{T}$}

% $\eta \gets \sqrt{\frac{R\cdot B \cdot T}{D_1}}$ \\ 
% $\textbf{costs} \gets \textbf{Unif}\left(\left[0, \eta\right], \mathbb{I}_{N\times N}\right)$ ,  \\ 
% \For{round $t=1,2,...,T$}{
% $x_t \gets M(costs)$ \\ 
% Observe sample $\hat r_t \sim \frac{1}{f} \textbf{Binom}(r_t,f,\mathbb{I}_{N\times N})$ \\
% $\textbf{costs} \gets \textbf{costs} + \hat r_t$
% }
% \label{alg:NFPL}
% \caption{Follow the Perturbed Leader with Uniform Noise (NFPL) for Caching}
% \end{algorithm}
% {\noindent}Algorithm \ref{alg:NFPL} only observes a sample of requests $\hat r_t$ such that each request is seen with probability $p$. This results in noisy frequency count.

==> Recovery_Files/approach2.tex <==
%\subsection{FPL with noisy costs}
\begin{algorithm}[t]
\KwIn{Set of decisions $\mathcal{X}$; Time Horizon $T$; $R, \; A, \; D$}
\KwOut{Sequence of decisions: $\{\mathbf{x_t}\}_{1}^{T}$}

$\eta \gets \sqrt{\frac{R\cdot A \cdot T}{D}}$ \\ 
$\hat{\textbf{costs}} \gets  0$ ,  \\ 
\For{round $t=1,2,...,T$}{
$\boldsymbol{\gamma}_t \sim \textbf{Unif}\left(\left[0, \eta\right]^{N}, \mathbb{I}_{N\times N}\right)$ \\
$\mathbf{x_t} \gets M(\hat{\textbf{costs}} +  \boldsymbol{\gamma}_t)$ \\ 
Observe $\hat{\mathbf{r_t}}$ \\
$\hat{\textbf{costs}} \gets \hat{\textbf{costs}} + \mathbf{\hat{r}_{t}}$
}
\caption{Noisy Follow the Perturbed Leader with Uniform Noise (NFPL)}
\label{alg:NFPL}
\end{algorithm}

In this section we introduce an extension to the general FPL algorithm, named \textit{Noisy Follow the Perturbed Leader} (NFPL), that does not have necessarily access to the exact cost vector $\mathbf{r}_t \in \bar{\mathcal{B}}$, but only to its estimation given by a general estimator $\mathbf{\hat r}_t$. We assume that $\mathbf{\hat r}_t$ is unbiased with bounded $l_1$ norm for every realization, i.e.,
%Our main contribution is proposing a more general version of the FPL algorithm where we do not have necessarily access to the exact cost vector, $r_t$, but only to its estimation: $\hat r_t$. $\hat r_t$ is an unbiased estimator of $r_t$ with bounded $l_1$ norm for every realization, i.e. 
\begin{align}
   \E{\mathbf{\hat r}_t} = \mathbf{r}_t , \; \exists \hat A \in \mathbb{R}^+ \; \text{s.t.} \; \sup_{\mathbf{\hat r} \in \mathcal{\hat B}} \norm{\mathbf{\hat r} (\omega)}_1 \leq \hat A,
\end{align}
%G: we could try to improve the names of the constants. For me it would be natural to have R for the bound on the requests and perhaps C for the scalar product r x which corresponds to the cost.
where, $\norm{\mathbf{r}}_1 = \sum_{i=1}^{N} |r_i|$, and $\mathcal{\hat B} \subseteq \mathbb{R}^N$ is the set of all the realizations of every possible vector in the cost set $\bar{\mathcal{B}}$. %all $\mathbf{r} \in \bar{\mathcal{B}}$, where $\bar{\mathcal{B}}$ is the set of all costs. %$\mathcal{\hat B} = \{\mathbf{\hat r}_t(\omega) : \omega \in \Omega\}$ where $\Omega$ is the set of all the realizations of $\mathbf{\hat r}_t$. 
To clearly describe the algorithm we also need to introduce the definition of the upper bound of the cost, and the diameter of the decision set $\mathcal{X} \subseteq \mathbb{R}^N$ as
\begin{align}
    &\hat R = \sup_{x\in \mathcal{X}, r \in \mathcal{\bar{\hat{B}}}} \scalar{r}{x},\\
    %G: \bar{\hat{B}} is not defined, should it be \hat{B}?
    &D= \sup_{x,y \in \mathcal{X}} \norm{x-y}_{1}.
%    &A = \sup_{r\in \bar{\mathcal{B}}} \norm{r}_{1} 
\end{align}

We highlight that NFPL is not specific just to online caching, but it can deal with any general online linear learning problem. %Indeed, as described in Algorithm~\ref{alg:NFPL}, NFPL receives in input the set of decisions $\mathcal{X}$ that can be any compact subset of $\mathbb{R}^N$ with $l_1$ diameter $D$. %; iii) the upper bound $A$ on the norm of any realization of the request estimator; iv) the upper bound $R$ on the cost and v) the diameter $D$ of the decision set. 
As described in Algorithm~\ref{alg:NFPL}, NFPL follows in the footsteps of FPL with uniform noise, but considers the estimation from $\mathbf{\hat r}_t$ instead of the real cost vector $\mathbf{r}_t$. In particular, at each time-slot $t$, the algorithm generates $\boldsymbol{\gamma}_t$ from a multivariate uniform distribution in $[0, \eta]^N$, and it updates the decision vector with the minimizer of $\scalar{\mathbf{x}}{\mathbf{\hat r}_{1:t-1} +  \boldsymbol{\gamma}_t}$ over $\mathbf{x} \in \mathcal{X}$. %, where $\hat{\textbf{costs}} = \mathbf{\hat r}_{1:t-1}$.  %Once the estimation is observed, the algorithm updates the cumulative cost. %with the estimation $\mathbf{\hat r}_t$. 
%We want to highlight that NFPL is not specific to the caching problem but it can deal with any general online learning problem. More specifically, the set of the decisions $\mathcal{X}$
%Our proposed algorithm $1$, we call it Noisy Follow the Perturbed Leader (NFPL),  follows the same procedure as FPL with uniform noise but using at each time step, the estimation $\hat r_t$ instead of the real cost vector $r_t$. Algorithm $1$ is not specific to the caching problem but more general to any online learning problem. More specifically, the set of decisions $\mathcal{X}$ could be any other compact set with $l_1$ diameter $D = \sup_{x,y \in \mathcal{X}} \norm{x-y}_{1}$. The set $\bar{\mathcal{B}}$ of costs could be any other with bounded $l_1$ norm for every one of its elements, 

The performance of NFPL in terms of regret, as defined in~\eqref{eq:pseudoregret}, is expressed by the following theorem. 
\begin{theorem}[Regret bound NFPL]
For $\eta = \sqrt{\frac{R\cdot A \cdot T}{D}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \bar{\mathcal{R}}_{T}(\text{NFPL}) \leq 2 \sqrt{\hat R\cdot \hat A \cdot D\cdot T}
        \end{align}
\end{theorem}

\begin{IEEEproof}
Let $\{r_t\}_{0}^{T}$ be sequence of costs and $\{\hat{r_t}\}_{0}^{T}$ a realization from the unbiased estimator.
   The cost of NFPL given $\{r_t\}_{0}^{T}$ and $\{\hat{r_t}\}_{0}^{T}$ is expressed as: 
    \begin{align}
        \text{NFPL}_{T} = \sum_{t=1}^{T} \scalar{r_t}{ M(\hat r_{0:t-1})}\ .
    \end{align}
We similarly define the policy $\hat{\text{NFPL}}$ that plays the same actions as NFPL,  but evaluated with respect to the noisy costs, more specifically its cost is given by: 

\begin{align}
   \hatname{NFPL}_{T} = \sum_{t=1}^{T} \scalar{\hat r_t} {M(\hat r_{0:t-1})}   \ . 
\end{align}
We define also $\hat{\text{OPT}}$, the minimum cost incurred under sequence $\{\hat{r_t}\}_{0}^{T}$ given by: 
\begin{align}
    \hat{\text{OPT}}_{T} = \scalar{\hat r_{1:T}}{M(\hat r_{1:T})}
\end{align}
We compute the regret of NFPL as follows:
%G: this is wrong (I had already written it on the pages I gave to Younes), the supremum is missing. You need to say that you do the calculation for a specific sequence r_t and then take the expectation
\begin{align}
    &\bar{\mathcal{R}}_{T}(\text{NFPL}) \\
&= \E{\text{NFPL}_{T} - \text{OPT}_{T}}  \\ 
&= \E{\text{NFPL}_{T} - \hatname{NFPL}_{T}} + \\
&\;  \E{\hatname{NFPL}_{T} - \hatname{OPT}_{T}} + \E{ \hatname{OPT}_{T} -\text{OPT}_{T}}
\end{align}
We have: 
\begin{align} \label{e:proof-NFPL1}
    &\E{\text{NFPL}_{T} - \hatname{NFPL}_{T}} =0\\ \label{e:proof-NFPL2}
    &\E{\hatname{OPT}_{T}-\text{OPT}_{T}} \leq 0 \\ \label{e:proof-NFPL3}
    &\E{\hatname{NFPL}_{T} - \hatname{OPT}_{T}} \leq 2\sqrt{\hat R\cdot \hat A\cdot D} \times \sqrt{T} 
\end{align}
The equality \eqref{e:proof-NFPL1} follows from the estimations of the noisy cost at each time step being independent, then in particular $\hat r_t$ and $\hat r_{0:t-1}$ are independent and thus $\E{\scalar{\hat r_t}{M(\hat r_{0:t-1})} } = \scalar{r_t}{M(\hat r_{0:t-1})}$. The inequality \eqref{e:proof-NFPL2} is because $\hatname{OPT}\leq \hat r_{1:T} M(r_{1:T}) $. The inequality \eqref{e:proof-NFPL3} follows from \cite[Theorem 1.1]{kalai2005efficient}. 
\end{IEEEproof}

\begin{remark}
FPL algorithm for online linear learning as presented in \cite{kalai2005efficient} has a regret
%G: is this expected regret or pseudo-regret? the relation with what is discussed here it unclear. is kalai2005efficient about FPL with known costs? If so, we should not say that we do worse as our constants boil down to theirs and we recover their result.
bound of $2\cdot \sqrt{R\cdot A \cdot D\cdot T}$ where $R =\sup_{x\in \mathcal{X}, r \in \mathcal{B}} \scalar{r}{x} $ and $A = \sup_{r\in \mathcal{B}}$.
%G: the definition of A is incomplete
It is easy to check that $\hat A\geq A$ and $\hat R \geq R$. It follows that the bound for FPL would be tighter than the one we proved. The trade-off is expressed by the ratio $\sqrt{\frac{\hat R \cdot \hat A }{R \cdot A}}$. 
\end{remark}

We now study three specific cases of the unbiased estimator in the online caching setting: i) $\mathbf{\hat r}_t = \mathbf{r}_t$, i.e., the estimator is deterministic and always correct in Section~\ref{ss:FPL-caching}; 
ii) the case where a fixed number of requests is sampled within each batch and  iii) the case where each request is sampled with a given probability in Section~\ref{ss:NFPL-Caching-Fixed}. 

\subsection{FPL for caching}
\label{ss:FPL-caching}
In the online caching problem, the case where $\mathbf{\hat r}_t = \mathbf{r}_t$ translates in dealing with the exact file requests. The following result applies to the online caching problem with batched requests. 
%We consider a particular case to adapt Algorithm~\ref{alg:NFPL} for the batched caching problem. The decisions set and the costs set will be as defined in Section~\ref{sec:bacground}. Moreover, we consider the deterministic case where the estimator $\hat{\mathbf{r_{t}}}$ is always exact, i.e. $\hat{\mathbf{r_t}} = \mathbf{r_t}$. We deduce then the following result: 
\begin{corollary} [Regret bound FPL caching] \label{co:FPL-uniform-noise}
Algorithm 1 applied for caching with exact requests has the following regret bound: 
\begin{align}
           \bar{\mathcal{R}}_{T}(\text{FPL})
& \leq 2\sqrt{2}\cdot  B \cdot \sqrt{C \cdot T}\ .
\end{align}
given that $C<N/2$.
\end{corollary}
\begin{IEEEproof}
We apply Theorem $1$ for the case where the decision set $\mathcal{X}$ is as in \eqref{eq:Capped-Simplex}, implying that the diameter $D$ is equal to $2\cdot C$ when $C<N/2$.
%G: isn't this always true also when C > N/2?
Also, the costs set $\bar{\mathcal{B}}$ is as in \eqref{eq:requests_set} and the unbiased estimator $\hat {\mathbf{r_t}}$ is always equal to the request $\mathbf{r_t}$. It follows that  $\mathcal{\bar{B}}= \hat{\mathcal{B}}$ and then, by definition of $\mathcal{\bar{B}}$, it follows that $\hat A=B$ and $\hat R=B$. Replacing the constants $\hat R, \hat A$ and $D$ in the result of Theorem $1$ we get our result. 
\end{IEEEproof}

In~\cite{bhattacharjee2020fundamental} Bhattacharjee et al. proposed an FPL-based algorithm with a Gaussian noise for the online caching problem and they proved the following bound on the regret (according to the regret definition in~\eqref{eq:regret}). 

\begin{theorem}\cite[Theorem 3]{bhattacharjee2020fundamental}
\label{th:FPL-gaussian-noise}
  For $\eta = \frac{1}{4\pi (\ln N)^{1/4}} \cdot \sqrt{\frac{T}{C}}$ and for $\gamma_t$ normal gaussians, with $r_0 = \eta \cdot \gamma_t$, the expected regret of FPL is given by: 
  \begin{align}
      \mathcal{R}_{T}(\text{FPL})  \leq 1.51 \cdot (\ln N)^{1/4} \cdot \sqrt{C\cdot T}\ .
  \end{align}
\end{theorem}

Since $\mathcal{\bar R}_T \le \mathcal{R}$ the regret bound is also valid for the weak regret defined in~\eqref{eq:pseudoregret}. In this view, our analysis presents two main novelties. First, our bound in Corollary~\ref{co:FPL-uniform-noise} is also valid in the case where the requests are batched, which is of practical interest since updating the cache at each request might be computationally impractical due to the high request rate. Second, even when the batch size $B$ is equal to 1, we provide a bound that does not depend on the catalogue size, and hence it will not diverge as $N$ goes to infinity. %Our analysis has advantage over state of the art FPL algorithm for caching in two dimensions. First, our bounds are also valid when requests are batched, which is of practical interest, since updating the cache at each time step might be unfeasible due to the high request rate. Second, even for the case when the batch size $B=1$, our regret bounds are tighter for a catalogue size $N\geq 13$. Moreover, \cite{bhattacharjee2020fundamental} bounds diverge as $N$ goes to infinity in contrast with our bounds that are independent of the catalogue size.

\subsection{NFPL for caching}
\label{ss:NFPL-Caching-Fixed}
In the caching problem, especially in cases where the request rate is very high~\cite{estan2002new}, the sample of the actual requests within each batch can allow the use of slower and cheaper memory. In what follows we take into account two different ways of sampling requests inside each batch of requests. First, we consider the case where the caching system samples a fixed number of requests from each batch. Second, we consider the case where each request of the batch is independently sampled with a specified probability.

{\noindent \textbf{Fixed number of samples}}. 
%For the caching problem, it is of interest to consider only a subset of requests at each batch of size $l<B$. This is beneficial as the rate by which counters are updated is smaller and hence it can be afforded to use a slower cheaper memory for storing counts for each object. 
%We consider then the setting where we have access a sample $l$ out of $B$ requests, chosen uniformly at random from the batch. If $s_t$ is the sequence of requests in the batch, with frequency count for each object inside the batch $r_t$, $\hat s_t$ is sub-sequence of $s_t$ with length $l<B$ and $\hat d_t$ is the frequency count for each object inside the batch $\hat s_t$ . The unbiased estimator in this case is given by: 
We study the setting where the caching system has access to a sample of $l < B$
%G: "b" instead of "l"?
requests uniformly chosen at random from the batch at each time-slot. Let $\mathbf{\hat d}_t$ denote the vector of requests for each file in the sampled batch. We then use the following unbiased estimator for $\mathbf{r}_t$:
\begin{equation}\label{e:fixed-batch}
        \mathbf{\hat{r}_{t}}  =   \frac{B}{l} \cdot  \mathbf{\hat{{d_t}}}: \; \E{\mathbf{\hat r_t}} = \mathbf{r_t}. \;
\end{equation}

Using NFPL in this setting, we obtain the following regret bound:
\begin{corollary}[Regret Bound NFPL with fixed size sub-batch]\label{co:NFPL-caching-fixed-subBatch}
      For $\eta = B \cdot \sqrt{\frac{T}{2\cdot C}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \bar{\mathcal{R}}_{T}(\text{NFPL}) \leq 2\sqrt{2} \cdot B \cdot \sqrt{C\cdot T}
        \end{align}
    
\end{corollary}
\begin{IEEEproof}
        We apply Theorem $1$ for the case where $\mathcal{X}$ is as in \eqref{eq:Capped-Simplex}, implying that the diameter $D$ is equal to $2\cdot C$ when $C<N/2$. Also, the costs set $\bar{\mathcal{B}}$ is as in \eqref{eq:requests_set} and the unbiased estimator $\hat {\mathbf{r_t}}$ is given in \eqref{e:fixed-batch}. Notice that in this case $\norm{\hat{\mathbf{r_t}}}_1 = B$ for every realization we deduce then that $\hat A = B$ and $\hat R = B$. Replacing the constants $\hat R, \hat A$ and $D$ in the result of Theorem $1$ we get our result. 
\end{IEEEproof}
\begin{remark}
The regret bound in Corollary \ref{co:NFPL-caching-fixed-subBatch} is independent from the sub-batch size $l$. However, we will show in Section~\ref{sec:experiments} that the smaller is the value of $l$, the higher is the variability in the cost of our algorithm.  
\end{remark}

{\noindent \textbf{Variable number of samples}}. Another approach is to consider a sub-batch where each request is independently sampled with probability $f>0$ at each iteration. In this case, the size of the sub-batch is a random variable and we consider the following unbiased estimator
%Another model, is to consider a sub-batch that samples each request with a probability $f>0$ at each time step, in this case the size of the batch is a random variable and the unbiased estimator $\hat r_t$ is expressed in this case as: 
\begin{equation}\label{e:estimator-rt-f}
    \mathbf{\hat {r}_t} = \frac{1}{f} \cdot \mathbf{\hat d}_t,
\end{equation}
where $\mathbf{\hat d}_t$ is defined as in \eqref{e:fixed-batch}. In this case, NFPL achieves the following regret bound:
\begin{corollary}[Regret Bound NFPL sampling probability $f$]\label{c:sampling}
      For $\eta = \frac{B}{f} \cdot \sqrt{\frac{T}{2\cdot C}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \mathcal{\bar{R}}_{T}(\text{NFPL}) \leq 2\sqrt{2} \cdot \frac{B}{f} \cdot \sqrt{C\cdot T}
        \end{align}
\end{corollary}
\begin{IEEEproof}
 We apply Theorem $1$ for the case where the decision set $\mathcal{X}$ is as in \eqref{eq:Capped-Simplex}, implying that the diameter $D$ is equal to $2\cdot C$ when $C<N/2$. Also, the costs set $\bar{\mathcal{B}}$ is as in \eqref{eq:requests_set} and the unbiased estimator $\hat {\mathbf{r_t}}$ is given in \eqref{e:estimator-rt-f}. Notice that in this case $\norm{\hat {\mathbf{r_t}}}_1 \leq \frac{B}{f}$ for very realization. It follows that $\hat A = \hat R = \frac{B}{f}$. Replacing the constants $\hat R, \hat A$ and $D$ in the result of Theorem $1$ we get our result. 
\end{IEEEproof}

\begin{remark}
    The bound in Corollary~\ref{c:sampling} shows the dependency on the sampling probability $f$. Surprisingly, we always have $\bar{\mathcal{R}}_{T} = \mathcal{O}(\sqrt{T})$ but as $f$ goes to $0$, the constant in our bound for the regret becomes larger.  
\end{remark}


% \begin{remark}
%  It seems that the difference between NFPL and FPL is the constant in the regret $\frac{1}{p}$. But NFPL has more variance, since the expectation is taken now over more randomness. 
% \end{remark}



% \begin{algorithm}[h] 
% \KwIn{$R,\; T,\; B, \; D_1$}
% \KwOut{Sequence of cached items: $\{x_t\}_{1}^{T}$}

% $\eta \gets \sqrt{\frac{R\cdot B \cdot T}{D_1}}$ \\ 
% $\textbf{costs} \gets \textbf{Unif}\left(\left[0, \eta\right], \mathbb{I}_{N\times N}\right)$ ,  \\ 
% \For{round $t=1,2,...,T$}{
% $x_t \gets M(costs)$ \\ 
% Observe sample $\hat r_t \sim \frac{1}{f} \textbf{Binom}(r_t,f,\mathbb{I}_{N\times N})$ \\
% $\textbf{costs} \gets \textbf{costs} + \hat r_t$
% }
% \label{alg:NFPL}
% \caption{Follow the Perturbed Leader with Uniform Noise (NFPL) for Caching}
% \end{algorithm}
% {\noindent}Algorithm \ref{alg:NFPL} only observes a sample of requests $\hat r_t$ such that each request is seen with probability $p$. This results in noisy frequency count.

==> Recovery_Files/background1.tex <==
We consider a single-cache system where requests for files are served locally by a cache of finite capacity or, in the case of file miss, by a remote server. This latter case implies a per-file dependent cost related to the file retrieval. Such a cost can represent the time needed to retrieve the file from the remote server, or a monetary cost due to the use of the network infrastructure. 
% Younes : Maybe it not necessary to specify the weights w_i  OK

{\noindent \bf Cache State}. The local cache has capacity $C \in \{1,\ldots,N\}$, and it stores the files entirely. The cache state at time $t$ is represented by the vector $\textbf{x}_t = [x_{t,i}]_{i\in \mathcal{N}}$ indicating the files missing in the cache, i.e., $x_{t,i} = 1$ if file $i$ is missing at time $t$. Such a vector belongs to the set
\begin{equation*}
\mathcal{X} = \left \{ x \in \{0,1\}^{N} | \sum_{i\in \mathcal{N}} x_{i} = N-C \right \}.
\end{equation*}
The set $\mathcal{X}$ is the capped simplex defined by the capacity constraint of the local cache.

{\noindent \bf Cache Updates}. Caching decisions are taken after  batch of $B$ requests has been cumulated, i.e., at each time-slot $t=1,\ldots,T$,
$B$ requests are collected from the users and the cache state is updated. The request process is represented as a sequence of vectors $\mathbf{r}_t = (r_{t,i} \in \mathbb{N}: i \in \mathcal{N})$ $\forall t$, where $r_{t,i}$ is the number of requests received for file $i$ at time $t$ in a file batch of size $B$. All the requests belong to the set
\begin{equation*}\label{eq:requests_set}
\mathcal{R} = \left \{ \mathbf{r}_t \in \mathbb{N}^N, t = 1, \dots, T | \sum_{i \in \mathcal{N}} r_{t,i} = B \right \}.
\end{equation*}
% Hence, we have
% \begin{equation}
%     \norm{\mathbf{r}_t}_{1} = B, \quad \norm{\mathbf{r}_t}_2 \leq B, \forall t \ .
% \end{equation}
{\noindent \bf Cost}. At each time-slot $t$, the caching system pays a cost equal to the number of requested files that are missing. Formally:
\begin{equation}\label{eq:cost}
\phi_{\mathbf{r}_t}(\mathbf{x}_t) = \scalar{\mathbf{r}_t}{\mathbf{x}_t}.
\end{equation}
% We have that: 
% \begin{align}
%     R &= \sup_{\mathbf{x},\mathbf{y}\in \mathcal{X}, t \in [T]} |\scalar{\mathbf{r}_t}{(\mathbf{x}-\mathbf{y})}| \leq B \cdot D_2 = \sqrt{2C}\cdot B \ .
% \end{align}
%Do we really need to define R ? 
For the sake of clarity, in what follows, for any vector $\mathbf{r}$, we indicate with $M(\mathbf{r})$ an arbitrary element of $\arg\min_{\mathbf{x}\in \mathcal{X}} \scalar{\mathbf{r}}{\mathbf{x}}$.
Furthermore, given a sequence of vectors $(\mathbf{r}_1, \dots, \mathbf{r}_t)$, we denote their aggregate sum as $\mathbf{r}_{1:t}\triangleq \sum_{s=1}^t \mathbf{r}_s$. 

\subsection{Online Caching}
Our caching problem falls in the \textit{Online Convex Optimization} framework~\cite{zinkevich2003online, hazan2016introduction}, where an agent (caching system) chooses an action $\textbf{x}_t$ from a convex set $\mathcal{X}$ at each time-slot $t$ before an adversary selects the cost function $\phi_{\mathbf{r}_t}$, i.e., the system changes the cache state before experiencing the cost. The cache state is determined by an online algorithm $\mathcal{A}$ that, at each time-slot $t$, computes the cache state $\textbf{x}_{t+1}$ for the next time-slot given the current state $\mathbf{x}_t$ and the costs seen so far $\{\mathbf{r}_{s}\}_{s=1}^{t}$. The main performance metric used to evaluate an online algorithm $\mathcal{A}$ is the regret:
%\begin{equation}\label{eq:regret}
%R_T(\mathcal{A}) = \sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{\sum_{t=1}^T %f_{\mathbf{r}_t}(\mathbf{x}_t) - \sum_{t=1}^T f_{\mathbf{r}_t}(\mathbf{x}^*) \right \}
%\end{equation}.
\begin{equation}\label{eq:regret}
    \mathcal{R}_T = \sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{\sum_{t=1}^{T} \scalar{\mathbf{r}_t}{\mathbf{x}_t} - \text{OPT}(1:T)\right \}.
\end{equation}
%Younes: Not sure if the point should be here, and I would prefer to mention x^{*} right away. 
This metric measures the difference the total cost incurred by $\mathcal{A}$ over a time horizon $T$ and the total cost of the static optimum $\text{OPT} = \scalar{\mathbf{r}_{1:T}}{M(r_{1:T})}$. %decision $\mathbf{x}^*$ in hindsight for any sequence of requests, i.e., $\mathbf{x}^* = \arg\min_{\mathbf{x} \in \mathcal{X}} \sum_{t=1}^T f_{\mathbf{r}_t}(\textbf{x})$. 
The supremum in~\eqref{eq:regret} indicates that the regret is compared against an adversary that generates requests trying to deteriorate the performance of the caching system.
% Younes: I do not know if maybe here we could talk about oblivious and adaptive, probably not the right place, because this only matters when the algorithm has randomness. I would also suggest to say instead that it holds for any sequence of requests. OK
In this setting, the main goal is the design of an online caching algorithm $\mathcal{A}$ that achieves sublinear regret, i.e., $R_T(\mathcal{A}) = o(T)$. This ensures that the designed algorithm behaves as the optimal static policy on average achieving zero average regret as $T$ increases.

\subsection{Follow the Perturbed Leader (FPL)}
In the OCO literature, one of the projection-free algorithms that achieve linear regret is the \textit{Follow the Perturbed Leader} (FPL) introduced by Vempala et al. in~\cite{kalai2005efficient}, and then studied in the caching framework by Bhattacharjee et al. in~\cite{bhattacharjee2020fundamental}.
%Younes: I would not say 0 regret  but sublinear regret. Most efficient might be a big claim. 
The algorithm is a smoothed version of the classic \textit{Follow the Leader} (FTL) algorithm~\cite{littlestone1994weighted} that greedily selects the next state minimizing the aggregate costs seen in the past, i.e., $x_{t+1}(\text{FTL}) = M(r_{1: t})$. %$\mathbf{x}_{t+1} = \arg\min_{\mathbf{x} \in \mathcal{X}} \sum_{\tau=1}^t f_{\mathbf{r}_{\tau}}(\mathbf{x})$. 
FTL algorithm is optimal when the cost functions are sampled from a stationary distribution, however, in the adversarial setting, the algorithm presents linear regret~\cite{de2014follow}. 
%The behaviour of FTL can be easily exploited by an adversary by always requesting all the files that are not stored in the current time-slot leading to a linear regret for the algorithm.
%Younes: Here we are talking about online convex optimization in general so I think it is a bit weird to go back to caching. I think maybe we could just cite a paper that shows FTL is not good OK

%Younes: Maybe this is the right time To introduce the notation M(r_{i:j}) OK
FPL algorithm improves the performance of FTL by adding an initial random noise vector $\mathbf{r}_0$ where each component of the vector is drawn from a uniform distribution independently. In this case, the update is the following:%in the range $\left[ -\eta , \eta\right]$ independently, where $\eta \in \mathbb{R}^+$. 
 \begin{equation}
     x_{t+1}(\text{FPL}) = M(r_{0:t}) \ .
 \end{equation}
As described in~\cite{bhattacharjee2020fundamental}, in the case of caching, the algorithm first samples a vector of random variables $\boldsymbol \eta$. Then, at every time-slot, it adds the random noise to 
the current cumulative cost vector $\mathbf{r}_{0:t}$. Finally, the algorithm caches $C$ files with the lowest perturbed cumulative cost at each time-slot.
As shown in~\cite{bhattacharjee2020fundamental}, FTPL provides optimal regret guarantees for the discrete caching problem. Furthermore, this algorithm is also computationally efficient with respect to other approaches such as \textit{Follow-the-Regularized-Leader} or the Online Gradient Descent (OGD) methods~\cite{paschos2020online}, since it requires a sorting operation instead of projection.
%Younes: Maybe here, we can just give the definition 
%Younes: We can here refer directly to OGD 




==> Recovery_Files/background2.tex <==
We consider a single-cache system in which file requests for a catalogue with $N$ files can either be served locally by a cache with finite capacity $C$ or, in the case of a file miss, by a remote server. 
%The latter scenario incurs a file-dependent cost associated with retrieving the file. This cost may represent the time needed to fetch the file from the remote server or a monetary expense due to the use of network infrastructure.
%G: WHY TALK ABOUT FILE-DEPENDENT COSTS IF LATER WE JUST LOOK AT THE MISS COST.

{\noindent \bf Cache State}. The local cache has a capacity $C \in \{1,\ldots,N\}$ and stores files in their entirety. The cache state at time $t$ is represented by the vector $\textbf{x}_t = [x_{t,i}]_{i\in \mathcal{N}}$, which indicates the files missing in the cache; that is, $x_{t,i} = 1$ if and only if file $i$ is not stored in the cache at time $t$. A feasible cache allocation is then represented by a vector in the set:

\begin{equation*}
\mathcal{X} = \left \{ x \in \{0,1\}^{N} | \sum_{i=1}^N x_{i} = N-C \right \}.
\end{equation*}

%The set $\mathcal{X}$ represents the capped simplex defined by the capacity constraint of the local cache.
%G: technically this is not the capped-simplex


{\noindent \bf Cache Updates}. Although caching policies are often assumed to update their state after each request, in high request regimes or when cache updates are computationally or communicationally expensive, the cache may update its state after receiving a batch of $B$ requests~\cite{salem2021no}.
We study caching policies in this more general setting and consider a time-slotted operation. At each time-slot $t=1,\ldots,T$,
$B$ requests are collected from the users and the cache state is updated. The request process is represented as a sequence of vectors $\mathbf{r}_t = (r_{t,i} \in \mathbb{N}: i \in \mathcal{N})$ $\forall t$, where $r_{t,i}$ is the number of requests received for file $i$ at time $t$ in a file batch of size $B$. All the requests belong to the set
\begin{equation*}\label{eq:requests_set}
\bar{\mathcal{R}} = \left \{ \mathbf{r}_t \in \mathbb{N}^N, t = 1, \dots, T | \sum_{i=1}^N r_{t,i} = B \right \}.
\end{equation*}

{\noindent \bf Cost}. At each time-slot $t$, the caching system pays a cost equal to the number file misses, i.e., the number of files that must be retrieved by the remote server. Formally:
\begin{equation}\label{eq:cost}
\phi_{\mathbf{r}_t}(\mathbf{x}_t) = \scalar{\mathbf{r}_t}{\mathbf{x}_t}= \sum_{i=1}^N r_{t,i} x_{t,i},
\end{equation}
where $\scalar{\mathbf{r}_t}{\mathbf{x}} \triangleq \sum_{i=1}^N r_{i} x_i$ denotes the scalar product of the two vectors $\mathbf{r}$ and $\mathbf{x}$.
% We have that: 
% \begin{align}
%     R &= \sup_{\mathbf{x},\mathbf{y}\in \mathcal{X}, t \in [T]} |\scalar{\mathbf{r}_t}{(\mathbf{x}-\mathbf{y})}| \leq B \cdot D_2 = \sqrt{2C}\cdot B \ .
% \end{align}
%Do we really need to define R ? 

For the sake of coinciseness, we introduce the following  notation. For any vector $\mathbf{r}$, we denote by $M(\mathbf{r})$ an arbitrary element of $\arg\min_{\mathbf{x}\in \mathcal{X}} \scalar{\mathbf{r}}{\mathbf{x}}$. Furthermore, given a sequence of vectors $(\mathbf{r}_1, \dots, \mathbf{r}_t)$, we represent their aggregate sum as $\mathbf{r}_{1:t}\triangleq \sum_{s=1}^t \mathbf{r}_s$.

\subsection{Online Caching}
%G: NO, THIS IS NOT TECHNICALLY CONVEX OPTIMIZATION, BECAUSE THE VARIABLE IS DISCRETE
Caching  may be framed as an \textit{online learning problem}~\cite{hazan2016introduction}, where an agent (the caching system) chooses an action $\textbf{x}_t$ from a set $\mathcal{X}$ at each time-slot~$t$ before an adversary selects the cost function $\phi_{\mathbf{r}_t}: \mathcal X \to \mathbb R$.
%, i.e., the system changes the cache state before experiencing the cost. 

The cache state is determined by an online algorithm $\mathcal{A}$ that, at each time-slot $t$, computes the cache state $\textbf{x}_{t+1}$ for the next time-slot given the current state $\mathbf{x}_t$ and the cost functions incurred so far, which, in our application, are  determined solely by the sequence of requests up to time~$t$, that is $\{\mathbf{r}_{s}\}_{s=1}^{t}$. 

The main performance metric used to evaluate an online algorithm $\mathcal{A}$ is the regret, for which two different definitions are available. The expected regret is defined as 
%\begin{equation}\label{eq:regret}
%\bar{\mathcal{R}}_T(\mathcal{A}) = \sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{\sum_{t=1}^T %f_{\mathbf{r}_t}(\mathbf{x}_t) - \sum_{t=1}^T f_{\mathbf{r}_t}(\mathbf{x}^*) \right \}
%\end{equation}.
\begin{equation}\label{eq:regret}
    \mathcal{R}_T(\mathcal A) = \E{\sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{\sum_{t=1}^{T} \scalar{\mathbf{r}_t}{\mathbf{x}_t} - \text{OPT}_T\right \}},
\end{equation}
where $\text{OPT}_T = \scalar{\mathbf{r}_{1:T}}{M(\mathbf{r}_{1:T})}$ is the minimum cost incurred under the request sequence $\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}$ by the optimal static allocation $\mathbf{x}^* = M(\mathbf{r}_{1:T})$, and the expectation is taken over all any random choice of the algorithm $\mathcal A$.
The expected regret quantifies then the performance gap over a time horizon $T$ between the algorithm $\mathcal{A}$  and best static cache allocation with hindsight.
%decision $\mathbf{x}^*$ in hindsight for any sequence of requests, i.e., $\mathbf{x}^* = \arg\min_{\mathbf{x} \in \mathcal{X}} \sum_{t=1}^T f_{\mathbf{r}_t}(\textbf{x})$. 
In contrast, the mean regret~\cite{belmega2018online} (also called pseudo-regret or weak regret) is defined as 
\begin{equation}\label{eq:pseudoregret}
    \bar{\mathcal{R}}_T(\mathcal A) = \sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{ \E{\sum_{t=1}^{T} \scalar{\mathbf{r}_t}{\mathbf{x}_t}} - \text{OPT}_T\right \}.
\end{equation}
The interpretation remains analogous, but the mean regret involves comparing the \emph{expected} performance of algorithm $\mathcal A$ with that of the optimal static cache allocation. Applying Jensen's inequality leads one directly to conclude that $\bar{\mathcal{R}}_T \le  \mathcal{R}_T$. Our findings are articulated in terms of the mean regret, which we will henceforth refer to as just 'regret'.

Due to the supremum over all request sequences in~\eqref{eq:regret} and in~\eqref{eq:pseudoregret}, regret metrics do not make any assumptions about the nature of the request sequence (e.g., no statistical regularity). This means that the request sequence could be generated by an adversary seeking to degrade the performance of the caching system.
% Younes: I do not know if maybe here we could talk about oblivious and adaptive, probably not the right place, because this only matters when the algorithm has randomness. I would also suggest to say instead that it holds for any sequence of requests. OK

In this setting, one aims for an algorithm with sublinear regret, $\bar{\mathcal{R}}_T(\mathcal{A}) = o(T)$. These algorithms are commonly known as \emph{no-regret algorithms} since their time-average cost approaches the optimal static policy's cost as $T$ grows.

%G: WRITE SOMETHING ALONG THE FOLLOWING LINES:
%Online algorithms have regret can achieve a regret bound of at most $\sqrt{T}$~\cite{mcmahan2017survey}. 
%G: exactly the opposite, this is a lower bound for caching problem (cite sinha, it has the probabilistic method proof we discussed). I am not sure such result is in mcmahan, as it is not true for general online learning algorithm (bandit algorithm can have \log t). I do not have time to check this, also because I think such bounds are in terms of the expected regret rather than the mean regret.
Various algorithms, such as Online Gradient Descent (OGD) and Follow the Regularized Leader (FRL), can attain $\mathcal O(\sqrt{T})$-regret for caching problems~\cite{paschos2019learning,mhaisen2022online}. However, their cache update procedures necessitate projecting a tentative solution back onto the feasible set, which incurs $O(N^2)$ computational cost~\cite{wang2015projection}. %in the general case~\cite{wang2015projection} of batched requests~\cite{salem2021no}. %and $O(...)$ for OGD and FRL, respectively~\cite{wang2015projection,}. 
%G: check the projection cost in Tareq, I think it is smaller.
In the next section, we present a lightweight caching algorithm with $O(\sqrt{T})$-regret.

\subsection{Follow the Perturbed Leader (FPL)}
In the online learning literature, one of the projection-free algorithms that achieve sublinear regret is the \textit{Follow the Perturbed Leader} (FPL) introduced by Vempala et al. in~\cite{kalai2005efficient}, and then studied in the caching framework by Bhattacharjee et al. in~\cite{bhattacharjee2020fundamental}.
The algorithm is a smoothed version of the classic \textit{Follow the Leader} (FTL) algorithm~\cite{littlestone1994weighted} that greedily selects the next state minimizing the aggregate costs seen in the past, i.e., $x_{t+1}(\text{FTL}) = M(r_{1: t})$. %$\mathbf{x}_{t+1} = \arg\min_{\mathbf{x} \in \mathcal{X}} \sum_{\tau=1}^t f_{\mathbf{r}_{\tau}}(\mathbf{x})$. 
FTL algorithm is optimal when the cost functions are sampled from a stationary distribution, however, in the adversarial setting, the algorithm presents linear regret~\cite{de2014follow}. 
%The behaviour of FTL can be easily exploited by an adversary by always requesting all the files that are not stored in the current time-slot leading to a linear regret for the algorithm.
%Younes: Here we are talking about online convex optimization in general so I think it is a bit weird to go back to caching. I think maybe we could just cite a paper that shows FTL is not good OK

%Younes: Maybe this is the right time To introduce the notation M(r_{i:j}) OK
FPL algorithm improves the performance of FTL by adding an initial random noise vector $\mathbf{r}_0$ where each component of the vector is drawn from a uniform distribution independently. In this case, the update is the following:
%Younes: FPL does not necessarily use a noise that is uniform or exponential, so we can keep it general ? Like by choosing the right noise ?
%in the range $\left[ -\eta , \eta\right]$ independently, where $\eta \in \mathbb{R}^+$. 
 \begin{equation}
     x_{t+1}(\text{FPL}) = M(r_{0:t}) \ .
 \end{equation}
As described in~\cite{bhattacharjee2020fundamental}, in the case of caching, the algorithm first samples a vector of random variables $\boldsymbol \eta$. Then, at every time-slot, it adds the random noise to 
the current cumulative cost vector $\mathbf{r}_{0:t}$. Finally, the algorithm caches $C$ files with the lowest perturbed cumulative cost at each time-slot.
As shown in~\cite{bhattacharjee2020fundamental}, FTPL provides optimal regret guarantees for the discrete caching problem. Furthermore, this algorithm is also computationally efficient with respect to other approaches such as \textit{Follow-the-Regularized-Leader} or the Online Gradient Descent (OGD) methods~\cite{paschos2020online}, since it requires a sorting operation instead of projection.
%Younes: Maybe here, we can just give the definition 
%Younes: We can here refer directly to OGD 




==> Recovery_Files/conclusions2.tex <==
In this paper we studied, in an online caching framework, a variant of the classic Follow-the-Perturbed-Leader (FPL) in the case of imperfect knowledge of the requests. First, we provided a general framework to analyse FPL in case of noisy requests and then we studied the performance of our proposed algorithm (NFPL) in terms of regret. We showed that NFPL achieves the same regret guarantees of FPL with perfect knowledge of the requests, as far the requests' estimates are unbiased. Second, we experimentally showed that in case of particular non-stationary requests,
NFPL outperforms classic caching policies. Furthermore, different sampling methods have similar performance in both synthetic and real datasets. Future works involve the study of other online algorithms with imperfect knowledge of requests in the online caching framework.

==> Recovery_Files/intro1.tex <==
The use of caching techniques is becoming pervasive in many research fields related to computer systems. Ranging from the speed-up of CPUs' performance to the optimization of users' experience in CDNs~\cite{bektas2007designing}. The main goal in a caching system
is to choose the set of files to be stored in the cache in order to maximize the 
probability that a new file request is served locally avoiding the file retrieval from a remote server. With the constant increasing of network traffic due to 
the diffusion of new services such as virtual and augmented reality applications~\cite{chatzopoulos2017mobile}, or edge video analytics~\cite{ananthanarayanan2017real}, caching policies can greatly help in mitigating the issues related to the transportation of data in computer networks.

Caching policies have been studied under different assumptions on the request process 
for new files. The most recent one belongs to the online learning theory where the 
requests are thought to be selected by an adversary~\cite{bhattacharjee2020fundamental,li2021online,paschos2019learning}. With this assumption, starting from the work of Paschos et al.~\cite{paschos2019learning}, the online caching has been analysed under the lens of the \textit{Online Convex Optimization} (OCO) framework~\cite{zinkevich2003online}. In this context, the main metric of interest is the \textit{regret}, i.e., the difference between the cost incurred by a given online algorithms
%algorithm not algorithms right ? 
and the cost of the best static solution that has complete knowledge of future requests over a fixed time horizon. The main goal is to design \textit{no-regret} algorithms, i.e., online policies whose regret grows sublinearly with the length of the time horizon~\cite{paschos2019learning}.

Several online caching policies have been proposed in the literature, based on well-known online algorithms such as Online Gradient Descent (OGD)~\cite{paschos2019learning}, Follow-the-Regularized Leader (FTRL) or Follow-the-Perturbed-Leader (FPL)~\cite{mhaisen2022optimistic}. All these policies assume to have perfect knowledge of the received requests, however, when the request rate is very high~\cite{estan2002new} it is hard to get the actual requests and the requests seen by the caching system can be noisy. In this case, online caching policies should perform a sampling of the actual requests. This can let the caching system afford to use cheaper and slower memory to serve the requests (e.g., the count-min sketch techniques). In this paper we consider the FPL algorithm (one of the computationally less expensive algorithms) in the caching context and we extend it to deal with noisy requests. We show that even when we do not have a perfect knowledge of the requests we can adapt FPL to have the same performance of the case with perfect knowledge as far as we have an unbiased estimator of the request process. To the best of authors' knowledge this is the first work that consider noisy request in the online caching framework.

In this work we propose an extension of FPL, namely Noisy-Follow-the-Perturbed-Leader (NFPL), able to work on batches of requests where the requests within each batch can be noisy. Our main contributions are the following:\\
{\noindent \it 1)} We study the FPL algorithm in a batched case of caching and we give a new bound that does not depend on the catalogue size.\\
{\noindent \it 2)} We extend FPL to work with noisy requests and we analytically prove that it provides the same performance with respect to the case with perfect knowledge in expectation as far as it has an unbiased estimator of the requests. \\
{\noindent \it 3)} We experimentally show, both on stationary traces and real ones, that NFPL present similar behaviour with respect to the classic FPL and LFU and it outperforms the state-of-the art in non-stationary cases.





==> experiments2.tex <==
\subsection{Experimental Settings}
\begin{figure}[t]
\centering
%\captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}
\begin{subfigure}{0.48\linewidth}
    \centering
    \includegraphics[width=0.99\linewidth]{FIGURES/Sampling Tradeoff Zipf.pdf}
\caption{Zipf $r=10^{6},\alpha = 1.0, B=200, M=2$}
\label{fig:occupancy-exp-c500-d1}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\linewidth}
  \centering
  \includegraphics[width=0.99\linewidth,keepaspectratio]{FIGURES/Sampling Tradeoff Akamai.pdf}
\caption{Akamai $r=2\times 10^{8}, N=1000, M=50  $}
\label{fig:occupancy-theory-c500-d1}
\end{subfigure}
\caption{Average Miss-Ratio vs. Sampling Probability}
\label{fig:occupancies}
\end{figure}  
{\bf 1) Datasets}: We evaluated the proposed approach on both synthetic and real datasets. \\
{\noindent \textit{Synthetic Data}}. We generate two kinds of synthetic traces sampled from a catalog of $N = 10^4$ files: the first one where file requests are i.i.d. and generated according to a \textit{Zipf} distribution with exponent $\alpha \in \{0.8,1.2,1.5\}$; the second trace is generated by requesting each file from the catalog in a \textit{round-robin} fashion, in this way all the files are uniformly distributed over all the requests. In the synthetic traces we fix a total of $10^5$ file requests, a batch size $B=200$ and a cache size $C \in \{100,200, 500\}$.\\
{\noindent \textit{Real Data}}. We tested also our solution on a real file request trace from the Akamai CDN provider~\cite{neglia2017access}. The trace recorded 1 week of file requests with a total number of $8.5 \times 10^7$ requests for a catalog of $N=10^3$ files.

{\bf 2) Online Algorithms}: Beyond the NFPL solution we implemented i) the basic FTL algorithm that acts as the classic LFU caching policy in the case of $B=1$; ii) FPL to show that NFPL has the same behaviour in different scenarios; iii) LRU caching policy that, in the face of a new request, it evicts the least recently requested file from the cache.

{\bf 3) Metric}: We compare all the algorithms with respect to the \textit{Average Miss Ratio}, i.e., the total cost over the first $t$ iterations, normalized by $Bt$. More formally, at each iteration $t$, the average miss ratio is given by
\begin{equation}
    \frac{1}{Bt}\sum_{\tau=1}^t \scalar{\mathbf{r}_{\tau}}{\mathbf{x}_{\tau}}.
\end{equation}

{\bf 4) Noisy Requests}. For the implementation of FNPL, we generate the noisy requests starting with original trace and sample the actual requests with a certain probability $p \in \{0.01, 0.5\}$. The case with $p = 1$ is equivalent to the FPL algorithm.

\subsection{Results}
In all the results, for the FPL-like algorithms we show the mean value of the average miss-ration over $M=50$ runs and we also show the variability over all the runs showing the $80\%$ of values up and above the mean. In what follows, we first compare NFPL against state-of-the-art solutions, and then we deepen the behaviour of the proposed algorithm with two different methods for sampling the requests.

{\noindent \bf NFPL vs. Classic Policies}. In Figure~\ref{fig:hit-rates} we compare the NFPL algorithm with respect to classic policies such as LRU, FTL and FPL for increasing cache size $C = 100, 200, 500$ over the \textit{round-robin} synthetic traces. For all the curves we show the average value of the cost over $M=50$ runs. For the FPL and NFPL curves we show also their variability over the runs. As we can notice from all the three sub-figure, in the round-robin setting the classic policies such as LRU and FTL (LFU for batched requests) are far from the optimal value, as expected (their values coincide). The NFPL with both the sampling-probability values is closer to the optimum with respect to FPL. This suggests that, in the case of a round-robin trace, where the requests are uniformly distributed over the time horizon, ignoring the actual requests can be beneficial, relying only on the randomness of the initial perturbation for the cache update.

{\noindent \bf Fixed vs. Variable number of samples}. Figure~\ref{fig:occupancies} shows the average miss-ratio of NFPL as the sampling probability increases in the synthetic trace with the Zipf distribution (Figure~\ref{fig:occupancy-exp-c500-d1}), and the Akamai trace (Figure~\ref{fig:occupancy-theory-c500-d1}). For the Zipf distribution we generated $10^6$ file requests, while for the Akamai trace we considered the first $2\cdot 10^8$ file requests. In both the figures we evaluated NFPL with two different cache sizes, i.e., $C \in \{10, 200\}$, and we implemented two variants for the sampling. The first one, \texttt{NFPL-Fix}, always samples a fixed sub-batch of requests for each batch of requests, while, the second variant, \texttt{NFPL-Var}, independently samples each request within each batch with a certain probability $f$. First, as expected, in both the synthetic and the real trace, the two variants of NFPL approach to their static optimum as the sampling probability increases (when the sampling probability is equal to $1$ the algorithm is equivalent to FPL). Secondly, we observe that the difference between the two sampling methods is very subtle. This implies that the sampling method does not significantly impact the performance of the proposed algorithm.
%FF: @Younes, we should specify the values used in the experiments for the fixed sub-batch (NFPL-Fix) and the probability of sampling f (NFPL-Var)
%FF: we should also change the name of the y-axis' label in all the plots ("Average Miss-Ratio) 



